Privacy-Preserving, Communication-Efficient, and Target-Flexible Hospital Quality Measurement

Integrating information from multiple data sources can enable more precise, timely, and generalizable decisions. However, it is challenging to make valid causal inferences using observational data from multiple data sources. For example, in healthcare, learning from electronic health records contained in different hospitals is desirable but difficult due to heterogeneity in patient case mix, differences in treatment guidelines, and data privacy regulations that preclude individual patient data from being pooled. Motivated to overcome these issues, we develop a federated causal inference framework. We devise a doubly robust estimator of the mean potential outcome in a target population and show that it is consistent even when some models are misspecified. To enable real-world use, our proposed algorithm is privacy-preserving (requiring only summary statistics to be shared between hospitals) and communication-efficient (requiring only one round of communication between hospitals). We implement our causal estimation and inference procedure to investigate the quality of hospital care provided by a diverse set of 51 candidate Cardiac Centers of Excellence, as measured by 30-day mortality and length of stay for acute myocardial infarction (AMI) patients. We find that our proposed federated global estimator improves the precision of treatment effect estimates by 59% to 91% compared to using data from the target hospital alone. This precision gain results in qualitatively different conclusions about the estimated effect of percutaneous coronary intervention (PCI) compared to medical management (MM) in 63% (32 of 51) of hospitals. We find that hospitals rarely excel in both PCI and MM, which highlights the importance of assessing performance on specific treatment regimens.

==> _federated_supplement_arxiv_section.tex <==
\section*{Overview of Supplementary Materials}
The supplement consists of four appendices. In Appendix I, we prove the data-adaptive property of the hospital-level weights. In Appendix II, we show how patient-level information is not required to solve for the data-adaptive hospital-level weights (i.e., summary-level information is sufficient). Appendix III and Appendix IV contain additional results from the simulation study and real data analysis, respectively.

\bigskip

\newpage
\spacingset{1.9} % DON'T change the spacing!


 \section*{Appendix I. Derivation of Influence Functions}
\subsection*{General Form of Influence Functions}
In this section, we summarize the general form of the influence functions for the target and source site estimators. The influence function in the target site $\xi_{i,T}^{(a)}$ is
\begin{align*}
    \sqrt{N}(\hat{\mu}^{(a)}_{T} - {\mu}^{(a)}_T) &= \frac{1}{\sqrt{N}} \sum_{i=1}^{N} \frac{I(R_i=T)}{\rho_T} \xi_{i,T}^{(a)} + o_p(1),
\end{align*}
where
\begin{align*}
    \xi_{i,T}^{(a)} &= \frac{I(A_i=a)Y_i}{\pi_a(X_i,\bga^*)} - \left(\frac{I(A_i=a)}{\pi_a(\bX_i;\bga^*)}-1\right)m_a(\bX_i;\bgb_a^*) - \mu_T^{(a)} \\
    &\quad+ D_1(\bga^*,\bgb_a^*) \phi_T(\bX_i;\bga^*) + D_2(\bga^*,\bgb_a^*) I_T \triangledown f(\bX_i,Y_i,\bgb_a^*),
\end{align*}
where $D_1(\bga^*,\bgb_a^*) = \E\left[(Y_i-m_a(\bX_i;\bgb_a^*)) (-\bX_i^\top \exp(\bga^{*\top} \bX_i) I(A_i=a))\right],$ \\
$D_2(\bga^*,\bgb_a^*) = \E\left[\bX_i^T \{\frac{I(A_i=a)}{\pi_a(\bX_i;\bga^*)} - 1\}\right]$, \\
$I_T = \E\left[\triangledown^2 L_T\right]^{-1} = \E\left[\triangledown^2\left[\frac{1}{N_T}\sum_{i=1}^{N_T} (Y_i - \bgb_a^\top \bX_i)^2\right]\right]^{-1} = \E\left[\frac{2}{N_T}\sum_{i=1}^{n_i} (\bX_i^T \bX_i)\right]^{-1}$, \\
$\phi_T(\bX_i;\bga^*) = \E\left[\bX_i^\top \pi_a(\bX_i;\bga^*) (1-\pi_a(\bX_i;\bga^*) \bX_i\right]^{-1} \{\bX_i^\top (I(A_i=a) - \pi_a(\bX_i;\bga^*) )\}$, \\
and $\triangledown f(\bX_i, Y_i, \bgb_a^*) = -2 \bX_i^\top (Y_i - \bgb_a^{*\top} \bX_i)$ for a linear outcome $Y_i$. When the outcome regression model is correctly specified, $D_1(\bga^*,\bgb_a^*) = 0$, and when the propensity score model is correctly specified, $D_2(\bga^*,\bgb_a^*) = 0$. \\

In the source sites, we must additionally consider estimation of the density ratio weights. Let $h(\bX_i;\bgg_k,\tau) = \bX_i \exp(\bgg_k^\top \bX_i) - \tau$, where $\bX = (1,X_1,...,X_p)^\top$ is a design matrix with $1$ in the first column and $\tau = (1, E_1(\bX))^\top$ is the covariate mean vector in the target population with $1$ in the first entry. By a Taylor series expansion, we can obtain that
\begin{align*}
    \sqrt{N}(\hat{\bgg}_k - \bgg_k^*) &= \frac{1}{\sqrt{N}\rho_k} \sum_{i=1}^N \Bigg\{H_1^{-1} h(\bX_i;\bgg_k^*,\tau^*) I(R_i=k) \\
    &\quad+ \sqrt{\frac{\rho_k}{\rho_T}}H_1^{-1}(\bX_i-\tau) I(R_i=T) \Bigg\} + o_p(1),
\end{align*}
where $H_1 = \E\left[-\bX_i \exp(\bgg_k^{*\top} \bX_i) \bX_i^\top\right]$. \\

Then the source site influence function is
\begin{align*}
    &\sqrt{N}(\hat{\mu}^{(a)}_k - {\mu}^{(a)}_k) \\
    &= \frac{1}{\sqrt{N}\rho_k} \sum_{i=1}^{N} \Bigg\{ I(R_i=T)m_a(\bX_i;\bgb_a^*) - \mu^{(a)}_k \\
    &\quad+ \left[Y_i -m_a(\bX_i;\bgb_a^*)\right] \left[\frac{I(R_i=k, A_i=a)\omega_k(\bX_i;\bgg_k^*)}{\pi_{a,k}(\bX_i;\bga_k^*)} + 2D_2^k(\bga_k^*,\bgb_a^*) I_k \bX_i \right]  \\
    &\quad+ D_1^k(\bga_k^*) IF_i(\bX_i;\bga_k^*) + D_1^k(\bgg_k^*) IF_i(\bX_i;\bgg_k^*) \Bigg\} + o_p(1),
\end{align*}
where
$D_{2}^k(\bga_k^*,\bgb_a^*) = \E \left[\bX_i^T \left(\frac{I(R_i=k,A_i=a)\omega_k(\bX_i;\bgg_k^*)}{\pi_{a,k}(\bX_i;\bga_k^*)}-1 \right) \right]$, \\
$I_k = \left[\E \triangledown^2 L_k (\bgb_a^*) \right]^{-1} = \left[\E\left( \frac{2}{n_k} \sum_{i=1}^{n_k} \bX_i^T \bX_i \right))\right]^{-1}$, \\
$D_{1,\bga_k^*}^k = \E \left[\{Y_i-m_a(\bX_i;\bgb_a^*)\} I(R_i=k, A_i=a) \exp(\bgg_k^{*^\top} \bX_i) \bX_i \frac{\pi_{a,k}(\bX_i;\bga_k^*)-1}{\pi_{a,k}(\bX_i;\bga_k^*)} \right]$, \\
$IF_i(\bX_i;\bga_k^*) = \left[\E(\bX_i^\top \pi_{a,k}(\bX_i;\bga_k^*)(1-\pi_{a,k}(\bX_i;\bga_k^*)) \bX_i \right]^{-1} \bX_i \cdot (I(A_i=a)-\pi_{a,k}(\bX_i;\bga_k^*))$, \\
$D_{1,\bgg_k^*}^k = \E \left[\{Y_i-m_a(\bX_i;\bgb_a^*)\} I(R_i=k, A_i=a) \bX_i \exp(\bgg_k^{*^\top} \bX_i) \frac{\exp(\bga^{*^\top} \bX_i)}{1+\exp(\bga^{*^\top} \bX_i)} \right]$, \\
$IF_i(\bX_i;\bgg_k^*) = H_1^{-1} h(\bX_i;\bgg_k^*,\tau^*)I(R_i=k) + \sqrt{\frac{n_k}{N_T}}H_1^{-1}I(R_i=T) (\bX_i-\tau)$.


\subsection*{Derivation of the Target Influence Function}
Suppose we have an estimator from the target site, $\hat{\mu}_{a,T}^T$ of the true $\mu_{a,T}$ for $a=0,1$. Suppose that the sample size in the target site is $N_T$. In the propensity score model, suppose that $\hat{\bga} - \bga^* = o_p(1)$. In the outcome regression model, suppose also that $\hat{\bgb_a} - \bgb_a^* = o_p(1)$. Then the influence function for $\hat{\mu}_{a,T}$ can be decomposed as

\begin{align*}
    \sqrt{N_T}\left(\hat{\mu}_{a,T}^T - \mu_{a,T}\right) &= \frac{1}{\sqrt{N_T}}\sum_{i=1}^{N_T} \left[\frac{I(A_i=a)Y_i}{\pi_a(X_i,\hat{\bga})} - \left(\frac{I(A_i=a)}{\pi_a(X_i,\hat{\bga})} - 1 \right) m_a(X_i,\hat{\bgb}_a) - \mu_{a,T} \right] \\
    &= \underbrace{\frac{1}{\sqrt{N_T}}\sum_{i=1}^{N_T}\left[\frac{I(A_i=a)Y_i}{\pi_a(X_i,\bga_k^*)} - \left(\frac{I(A_i=a)}{\pi_a(X_i,\bga_k^*)} - 1 \right) m_a(X_i,\bgb_a^*) - \mu_{a,T} \right]}_{T_1} \\
    &\quad+\underbrace{\frac{1}{\sqrt{N_T}}\sum_{i=1}^{N_T}\left[I(A_i=a)\left(\frac{1}{\pi_a(X_i,\hat{\bga})} - \frac{1}{\pi_a(X_i,\bga_k^*)}\right) \{Y_i - m_a(X_i,\bgb_a^*)\}   \right]}_{T_2} \\
    &\quad-\underbrace{\frac{1}{\sqrt{N_T}}\sum_{i=1}^{N_T}\left[ \left\{\frac{I(A_i=a)}{\pi_a(X_i,\bga_k^*)} - 1\right\}\{m_a(X_i,\hat{\bgb}_a)-m_a(X_i,\bgb_a^*)\} \right]}_{T_3} \\
     &\quad-\underbrace{\frac{1}{\sqrt{N_T}}\sum_{i=1}^{N_T}\left[I(A_i=a)\left(\frac{1}{\pi_a(X_i,\hat{\bga})}- \frac{1}{\pi_a(X_i,\bga_k^*)} \right) \{m_a(X_i,\hat{\bgb}_a)-m_a(X_i,\bgb_a^*)\} \right]}_{T_4}
\end{align*}


If either the outcome regression model or propensity score model is correctly specified, then $\E(T_1) = 0$. For $T_2$, when the outcome regression model is correctly specified but the propensity score model may be misspecified, $T_2 = o_p(1)$. To show this, note that since $\hat{\bga} \to \bga^*$, then $\frac{1}{\pi_a(X_i,\hat{\bga})}- \frac{1}{\pi_a(X_i,\bga^*)} = o_p(1)$. Let $D_i = I(A_i=a)\left(\frac{1}{\pi_a(X_i,\hat{\bga})} - \frac{1}{\pi_a(X_i,\bga^*)}\right) \{Y_i - m_a(X_i,\bgb_a^*)\}$. Given $X_i$, $i=1,...,N_T$, $D_i \perp D_j$ for $i \neq j$ and $\E(D_i \mid X_i) = 0$. Since $Var(D_i \mid X_i) \leq \max(\pi_i(\bga^*) - \pi_i(\hat{\bga}))^2 \to o_p(1)$, then for any $\epsilon>0$, by Chebyshev's inequality, $$P_{D|X}\left( |N_T^{-1/2} \sum_{i=1}^{N_T} D_i | \geq \epsilon \right) \leq \frac{Var(D_i \mid X_i)}{\epsilon^2} \leq o_p(1),$$ so $T_2 = o_p(1)$. But when the outcome regression model is misspecified, then $\E[Y-m_a(X,\bgb_a^*)] \neq 0$, and the uncertainty of $\hat{\bga}$ contributes to the uncertainty of $\hat{\mu}_{a,T}^T$, i.e., we need to consider the uncertainty contribution from the estimation of $\hat{\bga}$. By a similar argument, $T_3 = o_p(1)$ when the propensity score model is correctly specified. However, when it is misspecified, the influence function of $\hat{\bgb_a}$ must be considered as it will contribute to the influence function of $\hat{\mu}_{a,T}^T$. For $T_4$ to be $o_p(1)$, it suffices that the product $$\left\{{\pi_a(X_i,\hat{\bga})^{-1}}-{\pi_a(X_i,\bga^*)^{-1}} \right\} \cdot \{m_a(X_i,\hat{\bgb}_a)-m_a(X_i,\bgb_a^*)\}$$ be $O_p(n^{-d})$ where $d > 1/2$, which is easily satisfied if $\alpha$ and $\bgb_a$ are estimated by maximum likelihood, in which case the product converges at rate $O_p(n^{-1})$. In the general case where models may be misspecified, we need to plug-in the influence functions for $\hat{\bga}-\bga^*$ and $\hat{\bgb_a}-\bgb_a^*$.

Denote
$$g_0(X_i,\bga) := \frac{I(A_i=a)}{\pi_a(X_i,\bga)},$$ so that we can write $T_2$ as
\begin{align*}
    T_2 &= N_T^{-1/2} \sum_{i=1}^{N_T}\left[Y_i-m_a(X_i,\bgb_a^*)\right]\left[g_0(X_i,\hat{\bga})-g_0(X_i,\bga^*)\right] \\
    &= N_T^{-1/2} \sum_{i=1}^{N_T}\left[Y_i-m_a(X_i,\bgb_a^*)\right] \triangledown g_0(X_i,\bga^\prime)(\hat{\bga}-\bga^*) \\
    &= N_T^{-1/2} \sum_{i=1}^{N_T}\left[Y_i-m_a(X_i,\bgb_a^*)\right] \triangledown g_0(X_i,\bga^*)(\hat{\bga}-\bga^*) \\
    &\quad+ \underbrace{N_T^{-1/2} \sum_{i=1}^{N_T}\left[Y_i-m_a(X_i,\bgb_a^*)\right] \underbrace{\left[\triangledown g_0(X_i,\bga^\prime)- \triangledown g_0(X_i,\bga^*)\right]}_{o_p(\sqrt{N_T})} (\hat{\bga}-\bga^*)}_{o_p(1)} \\
    &= N_T^{-1} \sum_{i=1}^{N_T}\left[Y_i-m_a(X_i,\bgb_a^*)\right] \triangledown g_0(X_i,\bga^*) \cdot \sqrt{N_T}(\hat{\bga}-\bga^*) + o_p(1),
\end{align*}
where $||\bga^\prime-\bga^*|| < ||\hat{\bga}-\bga^*||$.

By the law of large numbers, $$N_T^{-1} \sum_{i=1}^{N_T}\left[Y_i-m_a(X_i,\bgb_a^*)\right] \triangledown g_0(X_i,\bga^*) \to \E\left[\left[Y_i-m_a(X_i,\bgb_a^*)\right] \triangledown g_0(X_i,\bga^*)\right] = D_1(\bgb_a^*,\bga^*).$$ Further assume that $\sqrt{N_T}(\hat{\bga}-\bga^*) = N_T^{-1/2} \sum_{i=1}^{N_T} \phi_T(\bX_i;\bga) $ where $\phi_T(\bX_i;\bga)$ is the influence function for $\hat{\bga}$. Then $$T_2 = N_T^{-1/2}\sum_{i=1}^{N_T}D_1(\bgb_a^*,\bga^*) \cdot \phi_T(\bX_i;\bga) + o_p(1).$$
If the outcome regression model is correctly specified, then $$D_1 = \E_{X,A}\{\triangledown g_0(X_i,\bga^*) \E_{Y|X,A}\left[Y_i-m_a(X_i,\bgb_a^*)\right]\} = 0,$$ and $T_2 = o_p(1)$.

Now focusing on $T_3$, we can write
\begin{align*}
    T_3 &= \frac{1}{\sqrt{N_T}}\sum_{i=1}^{N_T}\left[ \left\{\frac{I(A_i=a)}{\pi_a(X_i,\bga^*)} - 1\right\}\{m_a(X_i,\hat{\bgb}_a)-m_a(X_i,\bgb_a^*)\} \right] \\
    &= \frac{1}{\sqrt{N_T}}\sum_{i=1}^{N_T}\left[ \left\{\frac{I(A_i=a)}{\pi_a(X_i,\bga^*)} - 1\right\} \triangledown m_a(X_i,\bgb_a^*) (\hat{\bgb_a}-\bgb_a^*) \right] + o_p(1) \\
    &= N_T^{-1}\sum_{i=1}^{N_T} \left[ \left\{\frac{I(A_i=a)}{\pi_a(X_i,\bga^*)} - 1\right\}\triangledown m_a(X_i,\bgb_a^*)\right] \cdot \sqrt{N_T} (\hat{\bgb_a}-\bgb_a^*)  + o_p(1).
\end{align*}
By the law of large numbers, $$N_T^{-1}\sum_{i=1}^{N_T} \left[ \left\{\frac{I(A_i=a)}{\pi_a(X_i,\bga^*)} - 1\right\}\triangledown m_a(X_i,\bgb_a^*)  \right] \to \E\left[\left\{\frac{I(A_i=a)}{\pi_a(X_i,\bga^*)} - 1\right\}\triangledown m_a(X_i,\bgb_a^*)\right] = D_2(\bga^*,\bgb_a^*).$$
How do we estimate ${\bgb}_a$? Suppose $\bgb_a$ is estimated within each site so that $$\hat{\bgb_a}_k = \argmin_{\bgb_a} L_k(\bgb_a) = \argmin_{\bgb_a} n_k^{-1} \sum_{i=1}^{n_k} f(X_i,Y_i,\bgb_a),$$
for some specified loss function $f$. For example, $f(x,y,\bgb_a) = (y-\bgb_a^\top x)^2$ for linear regression, and $f(x,y,\bgb_a) = \log\{1+\exp(\bgb_a^\top x)\} - y \bgb_a^\top x$ for logistic regression.
By a Taylor series expansion of the gradient, $$0 = \triangledown L_k(\hat{\bgb_a}_k) = \triangledown L_k(\bgb_a^*) + \triangledown^2 L_k(\bgb_a')(\hat{\bgb_a}_k - \bgb_a^*),$$ where $||\bgb_a'-\bgb_a^*|| \leq ||\hat{\bgb_a}_k - \bgb_a^*||$. This implies that $$\sqrt{n_k} \E\triangledown^2L_k(\bgb_a^*) (\hat{\bgb_a}_k-\bgb_a^*) = \sqrt{n_k}\triangledown L_k(\bgb_a^*) + \underbrace{\sqrt{n_k}(\triangledown^2 L_k(\bgb_a')-\E \triangledown^2 L_k(\bgb_a^*)) (\hat{\bgb_a}_k-\bgb_a^*)}_{o_p(1)},$$
since $\triangledown^2 L_k(\bgb_a')- \E \triangledown^2 L_k(\bgb_a^*) = \underbrace{\triangledown^2 L_k(\bgb_a')-\triangledown^2 L_k(\bgb_a^*)}_{\text{by Lipschitz }C||\hat{\bgb_a}_k - \bgb_a^*|| \to O_p(n^{-1/2})} + \underbrace{\triangledown^2 L_k(\bgb_a^*) - \E \triangledown^2 L_k(\bgb_a^*)}_{\text{by Concentration } O_p(n^{-1/2})}.$

Thus, $$ \sqrt{n_k} (\hat{\bgb_a}_k - \bgb_a^*) = \sqrt{n_k} \{\E \triangledown^2 L_k(\bgb_a^*) \}^{-1} \triangledown L_k(\bgb_a^*) + o_p(1).$$
Denoting $\{E \triangledown^2 L_k(\bgb_a^*) \}^{-1}$ as $I_k$, we have
\begin{equation*}
    {\sqrt{n_k} (\hat{\bgb_a}_k - \bgb_a^*) = n_k^{-1/2}\sum_{i=1}^{n_k}I_k \cdot \triangledown f(x_i,y_i,\bgb_a) + o_p(1).}
\end{equation*}

If $\hat{\bgb}_a = \hat{\bgb}_{0a}$, using the outcome regression parameter fit in the target site, then $$\sqrt{N_T} (\hat{\bgb}_{0a} - \bgb_a^*) = N_T^{-1/2} \sum_{i=1}^{N_T} I_T \cdot \triangledown f(x_i,y_i,\bgb_a) + o_p(1).$$
Hence, we have $$T_3 = N_T^{-1/2}\sum_{i=1}^{N_T} D_2 \cdot I_T \cdot \triangledown f(x_i,y_i,\bgb_a) + o_p(1).$$
If the propensity score model is correctly specified, then $$D_2 = \E\left[ \left( \frac{I(A_i=a)}{\pi(X_i,\bga^*)} - 1 \right) \triangledown m_a(X_i,\bgb_a^*) \right] = 0,$$ and $T_3 = o_p(1).$ \\

Summarizing, since $T_4 = o_p(1)$, then combining $T_1$, $T_2$, and $T_3$, we obtain the influence function in the target site to be
\begin{align*}
    &\sqrt{N_T}(\hat{\mu}_{a,T}^T - {\mu}_{a,T}) \\
    &= \frac{1}{\sqrt{N_T}} \sum_{i=1}^{N_T} \Bigg\{\frac{I(A_i=a)Y_i}{\pi_a(X_i,\bga^*)} - \left(\frac{I(A_i=a)}{\pi_a(X_i,\bga^*)}-1\right)m_a(X_i,\bgb_a^*) - \mu_{a,T} \\
    &\quad+ D_1 \phi_T(x_i,\alpha) + D_2 I_T \triangledown f(X_i,Y_i,\bgb_a^*) \Bigg\} + o_p(1)
\end{align*}

When both outcome regression and propensity score models are correct, $D_1=D_2=0$, so the influence function reduces to
\begin{align*}
    &\sqrt{N}(\hat{\mu}_{a,T}^T - {\mu}_{a,T}) \\
    &= {\frac{1}{\sqrt{N}\rho_T} \sum_{i=1}^{N}I(R_i=T) \Bigg\{\frac{I(A_i=a)Y_i}{\pi_a(X_i,\bga^*)} - \left(\frac{I(A_i=a)}{\pi_a(X_i,\bga^*)}-1\right)m_a(X_i,\bgb_a^*) - \mu_{a,T} \Bigg\} + o_p(1).}
\end{align*}

When the outcome regression model is correct, but the propensity score model may be misspecified, $D_1=0$, so the influence function reduces to
\begin{align*}
    &\sqrt{N}(\hat{\mu}_{a,T}^T - {\mu}_{a,T}) \\
    &= {\frac{1}{\sqrt{N}\rho_T} \sum_{i=1}^{N}I(R_i=T) \Bigg\{ \{Y_i-m_a(X_i,\bgb_a^*)\} \left[\frac{I(A_i=a)}{\pi_a(X_i,\bga^*)} + 2D_2 I_T X_i \right] + m_a(X_i,\bgb_a^*) - \mu_{a,T} \Bigg\} + o_p(1)},
\end{align*}
since $\triangledown f(X_i,Y_i,\bgb_a^*) = 2X_i^\top(Y_i-m_a(X_i,\bgb_a^*))$.

When the propensity score model is correct, but the outcome regression model may be misspecified, $D_2=0$, so the influence function reduces to
\begin{align*}
    &\sqrt{N_T}(\hat{\mu}_{a,T}^T - {\mu}_{a,T}) \\
    &= \frac{1}{\sqrt{N_T}} \sum_{i=1}^{N_T} \Bigg\{\frac{I(A_i=a)Y_i}{\pi_a(X_i,\bga^*)} - \left(\frac{I(A_i=a)}{\pi_a(X_i,\bga^*)}-1\right)m_a(X_i,\bgb_a^*) - \mu_{a,T} + D_1 \phi_T(x_i,\alpha) \Bigg\} + o_p(1).
\end{align*}
It remains to obtain $\phi_T(x_i,\alpha)$. We follow the general strategy to find $\hat{\bga}$ that solves the system of moment equations, $E\left[h(X_i,\alpha)\right] = 0$. Since the system is exactly identified, the variance can be estimated as $\widehat{Var}(\hat{\bga}) = n^{-1}B^{-1}(\hat{\bga})M(\hat{\bga})B^{-1}(\hat{\bga})^\top$, where $B(\hat{\bga}) = -n^{-1}\sum_{i=1}^n \frac{\partial h(X_i,\alpha)}{\partial \alpha^\top} |_{\alpha=\hat{\bga}}$ and $M(\hat{\bga}) = n^{-1}\sum_{i=1}^n h(X_i,\hat{\bga}) h(X_i,\hat{\bga})^\top$. Based on M-estimation theory and the theory of influence functions, $\widehat{Var}(\hat{\bga}) = n^{-1}(n^{-1}\sum_{i=1}^n IF_i(\hat{\bga}) IF_i(\hat{\bga})^\top)$. It is clear that $$IF_i(\alpha) = \E\left[B(\alpha)\right]^{-1}h(X_i,\alpha).$$
For $\phi_T(x_i,\alpha)$ where the propensity score is estimated by logistic regression, $P(A_i=1 \mid X_i) = \pi_a(X_i,\alpha) = \frac{\exp(\alpha^\top x)}{1+\exp(\alpha^\top x)}$. Then $h(X_i,\alpha)=X_i^\top (A_i-\pi_a(X_i,\alpha))$ and $\frac{\partial h(X_i,\alpha)}{\partial \alpha^\top} = -X_i^\top \left[\pi_a(X_i,\alpha)(1-\pi_a(X_i,\alpha))\right] X_i$. Hence $$\phi_T(X_i,\alpha) = E\left[X_i^\top \pi_a(X_i,\alpha)(1-\pi_a(X_i,\alpha))X_i\right]^{-1} \cdot X_i^\top (I(A_i=a)-\pi_a(X_i,\alpha)).$$

The influence function $\sqrt{N}(\hat{\mu}_{a,T}^T - {\mu}_{a,T})$ reduces to
\begin{align*}
    \sqrt{N}(\hat{\mu}_{a,T}^T - {\mu}_{a,T})
    &= \frac{1}{\sqrt{N}\rho_T} \sum_{i=1}^{N}I(R_i=T) \Bigg\{ \underbrace{\left(\frac{I(A_i=a)Y_i}{\pi_a(X_i,\bga^*)} - \mu_{a,T} \right)}_{\text{Mean } 0} \\
    &\quad- \underbrace{\left(\frac{I(A_i=a)}{\pi_a(X_i,\bga^*)}-1\right) \cdot \Big[m_a(X_i,\bgb_a^*) + G_1 G_2^{-1} \pi_a(X_i,\bga^*)X_i^\top \Big]  \Bigg\}}_{\text{Mean } 0 \text{ under correct PS model}} + o_p(1),
\end{align*}

where $$G_1 = \E\left[\left[Y_i-m_a(X_i,\bgb_a^*)\right]I(A_i=a)\frac{X_i(\pi_a(X_i,\bga^*)-1)}{\pi_a(X_i,\bga^*)} \right]$$ and $$G_2 = \E\left[X_i^\top\pi_a(X_i,\bga^*)(1-\pi_a(X_i,\bga^*))X_i\right].$$


\subsection*{Source Sites}
In the source sites, we must additionally consider estimation of the density ratio weights. Let $h(X_i,\bgg_k,\tau) = X_i \exp(\bgg_k^\top X_i) - \tau$, where $X = (1,X_1,...,X_p)^\top$ is a design matrix with $1$ in the first column and $\tau = (1, E_T(X))^\top$ is the covariate mean vector in the target population with $1$ in the first entry.
\begin{align*}
    0 &= n_k^{-1} \sum_{i=1}^{n_k} h(X_i,\hat{\gamma}_k,\hat{\tau}) \\
    &= \frac{1}{\sqrt{n_k}}  \sum_{i=1}^{n_k} h(X_i,\bgg_k^*,\tau^*) + n_k^{-1} \sum_{i=1}^{n_k} \triangledown_{\bgg_k} h(X_i,\bgg_k^\prime, \tau^\prime) \cdot \sqrt{n_k} (\hat{\gamma}_k - \bgg_k^*) \\ &\quad+ n_k^{-1} \sum_{i=1}^{n_k} \triangledown_{\tau} h(X_i,\bgg_k^\prime,\tau^\prime) \cdot \sqrt{n_k}(\hat{\tau}-\tau^*) + o_p(1) \\
    &\to \frac{1}{\sqrt{n_k}}  \sum_{i=1}^{n_k} h(X_i,\bgg_k^*,\tau^*) + \E\left[ \triangledown_{\bgg_k} h(X_i,\bgg_k^\prime, \tau^\prime) \right] \cdot \sqrt{n_k} (\hat{\gamma}_k - \bgg_k^*) \\ &\quad+ \E\left[ \triangledown_{\tau} h(X_i,\bgg_k^\prime,\tau^\prime) \right] \cdot \sqrt{n_k}(\hat{\tau}-\tau^*) + o_p(1)
\end{align*}
Re-arranging for $\sqrt{n_k}(\hat{\gamma}_k - \bgg_k^*)$,
\begin{align*}
    \sqrt{n_k}(\hat{\gamma}_k - \bgg_k^*) &= \frac{1}{\sqrt{n_k}}  \sum_{i=1}^{n_k} H_1^{-1} h(X_i,\bgg_k^*,\tau^*) + H_1^{-1}\sqrt{n_k} (\hat{\tau}-\tau^*) \\
    &= \frac{1}{\sqrt{n_k}}  \sum_{i=1}^{n_k} H_1^{-1} h(X_i,\bgg_k^*,\tau^*) + \sqrt{\frac{\rho_k}{\rho_T}} H_1^{-1}\sum_{i=1}^N \left[I(R_i \in T) (X_i-\tau)\right],
\end{align*}
where $H_1 = \E\left[-\triangledown_{\bgg_k} h(X_i,\bgg_k^*,\tau^*)\right]$.

Then
\begin{align*}
    \sqrt{N} (\hat{\gamma}_k - \bgg_k^*) &= \frac{1}{\sqrt{N}\rho_k} \sum_{i=1}^N \Bigg\{H_1^{-1} h(X_i,\bgg_k^*,\tau^*) I(R_i=k) + \sqrt{\frac{\rho_k}{\rho_T}}H_1^{-1}(X_i-\tau) I(R_i \in T) \Bigg\} + o_p(1),
\end{align*}
where $H_1 = \E\left[-X \exp(\bgg_k^{*^\top} X) X^\top\right]$.

To summarize, when the outcome regression model, propensity score model, and density ratio model are all correctly specified, then
\begin{align*}
    \sqrt{N}(\hat{\mu}_{a,T}^r - {\mu}_{a,T}) &= \frac{1}{\sqrt{N}\rho_k} \sum_{i=1}^N  \Bigg\{ I(R_i=T) m_a(X_i,\bgb_a^*) - \mu_{a,T} \\ &\quad+ \frac{I(R_i=k, A_i=a) \omega_k(X_i,\bgg_k^*)}{\pi_a(X_i,\bga^*)} \left[Y_i - m_a(X_i,\bgb_a^*)\right]  \Bigg\}  + o_p(1)
\end{align*}

When only the outcome regression model is correctly specified, then

\begin{align*}
    &\sqrt{N}(\hat{\mu}_{a,T}^r - {\mu}_{a,T}) \\
    &= \frac{1}{\sqrt{N}\rho_k} \sum_{i=1}^{N} \Bigg\{ I(R_i=T)m_a(X_i,\bgb_a^*) - \mu_{a,T} \\ &\quad+ \{Y_i-m_a(X_i,\bgb_a^*)\} \left[\frac{I(R_i=k, A_i=a)\omega_k(X_i,\bgg_k^*)}{\pi_a(X_i,\bga^*)} + 2D_2^r I_k X_i \right] \Bigg\} + o_p(1),
\end{align*}
where $D_2^r = \E\left[\left(\frac{I(A_i=a,T_i=k)\omega_k(X_i,\bgg_k^*)}{\pi_a(X_i,\bga^*)} - 1 \right)\triangledown m_a(X_i,\bgb_a^*) \right]$ and $I_k = \left[\E(\triangledown^2 L_k(\bgb_a^*))\right]^{-1}$.

When the propensity score model and density ratio model are correctly specified but the outcome regression model may be misspecified, then
\begin{align*}
    &\sqrt{N}(\hat{\mu}_{a,T}^r - {\mu}_{a,T}) \\
    &= \frac{1}{\sqrt{N}\rho_k} \sum_{i=1}^{N} \Bigg\{ I(R_i=T)m_a(X_i,\bgb_a^*) - \mu_{a,T} + \frac{I(R_i=k, A_i=a)\omega_k(X_i,\bgg_k^*)}{\pi_a(X_i,\bga^*)} \left[Y_i -m_a(X_i,\bgb_a^*)\right] \\
    &\quad+ \underbrace{\E \left[\{Y_i-m_a(X_i,\bgb_a^*)\} I(R_i=k, A_i=a) \exp(\bgg_k^{*^\top}X_i)\frac{\pi_a(X_i,\bga^*)-1}{\pi_a(X_i,\bga^*)} \right]}_{D_{1,\bga^*}^r} \\
    &\quad \cdot \underbrace{\left[\E(X_i^\top \pi_a(X_i,\bga^*)(1-\pi_a(X_i,\bga^*))X_i \right]^{-1}X_i \cdot (I(A_i=a)-\pi_a(X_i,\bga^*))}_{IF_i(X_i,\bga^*)} \\
    &\quad+ \underbrace{\E \left[\{Y_i-m_a(X_i,\bgb_a^*)\} I(R_i=k, A_i=a) X_i \exp(\bgg_k^{*^\top}X_i) \frac{\exp(\alpha^{*^\top}X_i)}{1+\exp(\alpha^{*^\top}X_i)} \right]}_{D_{1,\bgg_k^*}^r} \\
    &\quad \cdot \underbrace{H_1^{-1} h(X_i,\bgg_k^*,\tau^*)I(R_i=k) + \sqrt{\frac{n_k}{N_T}}H_1^{-1}I(R_i= T) (X_i-\tau)}_{IF_i(X_i,\bgg_k^*)} \Bigg\} + o_p(1).
\end{align*}

\section*{Appendix II. Data-Adaptive Weights}
In this section, we prove that given a suitable choice for $\lambda$, then $\hat{\eta}_k = \argmin_{\eta_k} \hat{Q}_a(\boldsymbol{\eta})$ are adaptive weights such that  $\hat{\eta}_k - \eta_k^* = O_p(n_k^{-1/2})$ when $\bar{\delta}_k = 0$ and $P(\hat{\eta}_k = 0) \to 1$ when $\bar{\delta}_k \neq 0$. Recall that
\begin{equation} \label{eq:l1}
    \hat{Q}_a(\boldsymbol{\eta}) = \sum_{i=1}^N \left[ \hat{\xi}^{(a)}_{i,T} - \sum_{k \in S} \eta_k( \hat{\xi}^{(a)}_{i,T} -  \hat{\xi}_{i,k}^{(a)} - \hat{\delta}_k)\right]^2 + \lambda \sum_{k \in S} |\eta_k|\hat{\delta}_k^2,
\end{equation}

First consider the case when $\bar{\delta}_k = 0$. Then the $\hat{Q}_a(\boldsymbol{\eta})$ function reduces to the sum of the squared error term. By the Central Limit Theorem, the normalized and centered estimator converges in distribution to a mean $0$ normal distribution with asymptotic variance $\Sigma$ given by $$ \Sigma = \E\left[ \hat{\xi}^{(a)}_{i,T} - \sum_{k \in S} \eta_k( \hat{\xi}^{(a)}_{i,T} -  \hat{\xi}_{i,k}^{(a)} - \hat{\delta}_k)\right]^2.$$
Solving for the minimizer of this asymptotic variance gives $\eta_k^*$, 
\begin{align*}
    0 &= \frac{\partial \Sigma}{\partial \eta_k} = 2 \eta_k \E\left[\xi^{(a)}_{i,T} - \xi^{(a)}_{i,k}\right]^2 + 2\E\left[\xi^{(a)}_{i,T}(\xi^{(a)}_{i,k}-\xi^{(a)}_{i,T})\right] \\
    & \implies \eta_k^* = \frac{\E\left[\xi^{(a)2}_{i,T} - \xi^{(a)}_{i,T}\xi^{(a)}_{i,k}\right]}{\E\left[\xi^{(a)}_{i,k}-\xi^{(a)}_{i,T}\right]^2} \\
    &\quad \quad \quad \quad= \frac{\E\left[\xi^{(a)2}_{i,T}\right]}{\E\left[\xi^{(a)}_{i,k}-\xi^{(a)}_{i,T}\right]^2}
\end{align*}
since $\xi^{(a)}_{i,T}$ and $\xi^{(a)}_{i,k}$ are independent and $E\left[\xi^{(a)}_{i,T}\right] = 0$.

Now consider the case when $\bar{\delta}_k \neq 0$. The asymptotic variance is given by $$\E\left[\xi^{(a)}_{i,T} - \sum_{k=1}^K \eta_k(\xi^{(a)}_{i,T}- \xi^{(a)}_{i,k}) - \hat{\delta}_k)\right]^2 + \lambda \sum_{k=1}^K |\eta_k|\hat{\delta}_k^2.$$
For simplicity, consider the case where there are two sites in total, with one target site and one source site. Taking the derivative of the asymptotic variance with respect to $\eta_k$, we obtain 

\begin{align*}
    0 &= 2 \eta_k \E\left[\xi^{(a)}_{i,T}-\xi^{(a)}_{i,k} - \hat{\delta}_k\right]^2 + 2\E\left[\xi^{(a)}_{i,T}(\xi^{(a)}_{i,T}-\xi^{(a)}_{i,k} - \hat{\delta}_k)\right] \\
    &\implies \eta_k^* = 
  \frac{\E\left[\xi^{(a)2}_{i,T}\right] + 1/2 \lambda \hat{\delta}_k^2 }{\E\left[\xi^{(a)}_{i,T}-\xi^{(a)}_{i,k} - \hat{\delta}_k\right]^2}.
\end{align*}

Then this can be estimated by $$\hat{\eta}_k = \frac{\sum_{i=1}^n \hat{\xi}^{(a)2}_{i,T} + \lambda \hat{\delta}_k^2 /2n_k}{\sum_{i=1}^n \left[\hat{\xi}^{(a)}_{i,T} - \hat{\xi}^{(a)}_{i,k}\right]^2 + n \hat{\delta}_k^2},$$
where it can be seen that $Pr(\hat{\eta}_k = 0) \to 1$ as $n_k \to \infty$ if $\hat{\delta}_k \neq 0$.

\section*{Appendix II. Privacy-preserving Penalized Regression}
In this section, we show that in the federated setting, we can solve for the $\eta_k$ that minimizes the $Q_a(\boldsymbol{\eta})$ function without sharing patient-level information from the influence functions. Recall that $\xi^{(a)}_{i,T}$ is the influence function for the target site and $\xi^{(a)}_{i,k}$ is the influence function for source site $k$ such that
\begin{align*}
    \sqrt{N}(\hat{\mu}^{(a)}_{j} - \mu^{(a)}_{T}) &= \frac{1}{\sqrt{N}}\sum_{i = 1}^N \xi^{(a)}_{i,T} + o_p(1), \\
    \sqrt{N}(\hat{\mu}^{(a)}_{k} - \mu^{(a)}_{k}) &= \frac{1}{\sqrt{N}}\sum_{i=1}^N \xi^{(a)}_{i,k} + o_p(1),
\end{align*}
 
To estimate $\eta_k$, we minimized a weighted $\ell_1$ penalty function,
\begin{equation} 
    \hat{Q}_a(\boldsymbol{\eta}) = \sum_{i=1}^N \left[ \hat{\xi}^{(a)}_{i,T} - \sum_{k \in S} \eta_k( \hat{\xi}^{(a)}_{i,T} -  \hat{\xi}_{i,k}^{(a)} - \hat{\delta}_k)\right]^2 + \lambda \sum_{k \in S} |\eta_k|\hat{\delta}_k^2,
\end{equation}
where $\eta_k \geq 0$ and $\sum_{k=1}^K \eta_k = 1$, $\hat{\delta}_k = \hat{\mu}^{(a)}_{k} - \hat{\mu}^{(a)}_{T}$ is the estimated bias from source site $k$, and $\lambda$ is a tuning parameter.

To see that patient-level influence function information is not required, denote $$\tilde{Y}_i = \hat{\xi}_{i,T}^{(a)}, \quad \tilde{\bX}_{i,k} = \hat{\xi}_{i,T}^{(a)}-\hat{\xi}_{i,k}^{(a)} - \hat{\delta}_k.$$
Then the first term of (\ref{eq:l1}) can be written as 
\begin{align*}
    (\tilde{Y} - \tilde{\bX} \eta_k)^\top (\tilde{Y} - \tilde{\bX} \eta_k) &= \tilde{Y}^\top \tilde{Y} + \eta_k^\top \tilde{\bX}^\top \tilde{\bX} \eta_k - 2 \eta_k^\top \tilde{\bX}^\top \tilde{Y} \\
    &= \underbrace{\sum_{k=1}^K \tilde{Y}_k^\top \tilde{Y}_k}_{S_{\tilde{Y}}} + \underbrace{\eta_k^\top \sum_{k=1}^K \tilde{\bX}_k^\top \tilde{\bX}_k \eta_k}_{S_{\tilde{\bX}}} - \underbrace{2 \eta_k^\top \sum_{k=1}^K \tilde{\bX}_k^\top \tilde{Y}_k}_{S_{\tilde{\bX Y}}},
\end{align*}
where $S_{\tilde{Y}}$ is a scalar, $S_{\tilde{\bX}}$ is a $p \times p$ matrix, and $S_{\tilde{\bX Y}}$ is a $1 \times p$-vector. Thus, it suffices to share only $S_{\tilde{Y}}$, $S_{\tilde{\bX}}$, and $S_{\tilde{\bX Y}}$ with the leading site.

\section*{Appendix III. Additional Simulation Study Results}
Recall that in the simulation study, we considered five settings with $K \in \{10, 20, 50\}$ total hospitals, and five estimators for the first wave simulation: one estimator using data from the target hospital only (Target-Only), two estimators using all sites that weights each site proportionally to its sample size (SS (naive), SS), and two estimators that employ the federated algorithm with alternative solvers (global-$\ell_2$, global-$\ell_1$). In the second wave simulation about direct standardization, we compare the federated algorithm with the fixed-effects regression, where fixed-effects regression refers to fitting a linear regression with $\E[Y|A, X, R] = \sum_{k = 1}^K\beta_{0k}I(k = R) + \sum_{k = 1}^K\beta_{Ak}I(k = R)A + X\boldsymbol{\beta}$.

\subsection*{Distribution of observations}
In the dense data setting of the first wave simulation, $\mathcal{D}_{\text{dense}}$, for the target hospital $k = 1$, for $p = 1, ..., P$, we let the location parameter $\Xi_{1p} = 0.15 + 0.05\frac{1-p}{P-1}$, the scale parameter $\Omega_{1p} = 1$, and the skewness parameter $\mathrm{A}_{1p} = 0$. For source hospitals $k = 2, ..., K$, if the sample size is greater than or equal to the third quartile, $n_k \geq \text{Q3}(\{n_k\}_{k = 1}^K)$, we set $\mathrm{A}_{kp} = 3\times 2/P$. If the sample size is less than or equal to the first quartile, $n_k \leq \text{Q1}(\{n_k\}_{k = 1}^K)$, we set $\mathrm{A}_{kp} = -1\times 2/P$. If the sample size is greater than the first quartile and less than the third quartile, $n_k \in (\text{Q1}(\{n_k\}_{k = 1}^K), \text{Q3}(\{n_k\}_{k = 1}^K))$, we set $\mathrm{A}_{kp} = 0$, which are the same as the parameters of the target hospital. 
In the sparse data setting, $\mathcal{D}_{\text{sparse}}$, we keep the location parameter $\Xi_{1p} = 0.15 + 0.05\frac{1-p}{P-1}$, the scale parameter $\Omega_{1p} = 1$. For the source hospitals, if the sample size is greater than or equal to the $65 - K/10$ quantiles, or less than or equal to the $35 + K/10$ quantiles, we set $\mathrm{A}_{kp} = 2$ for $p = 1, 2$, and $\mathrm{A}_{kp} = 0$ for the remaining source hospitals and the target hospital. 
For $P = 10$, besides the two continuous covariates coming from the $P = 2$ settings, the rest covariates are generated from Bernoulli distributions with mean $\theta_{kp} = 0.45 + 0.1\frac{p-3}{7}$, where $p = 3, ..., 10$, for all the source hospitals and $\theta_{kp} = 0.5$ for the target hospital.
We plot the observations in target and source hospitals for the $\mathcal{D}_{\text{dense}}$ and $\mathcal{D}_{\text{sparse}}$ data generating mechanisms when $K = 10$ and $P = 2$.

In the second wave simulation where direct standardization is considered, we focus on comparison between federated algorithm and fixed-effects regression. We consider two settings with the same covariate distribution, only differing in their true ATEs. In the first setting, the true ATEs are uniform in all the hospitals. While in the second setting, the true ATEs vary across the hospitals.

\begin{figure}[H]

    \centering
\includegraphics[scale = 0.4]{graphics/Figure1S_dense.pdf} 
\includegraphics[scale = 0.4]{graphics/Figure1S_sparse.pdf}
\caption{Red (black) dots are target (source) site observations ($K = 10$, $P = 2$). (Left) Dense covariate setting. (Right) Sparse covariate setting. }
    \label{fig:Xdist}
\end{figure}

\subsection*{Alternative number of covariates and distributions}
In the main text, Table 1 reported simulation results for $\mathcal{D}_{\text{sparse}}$ in Specifications I--V when $P = 2$ covariates across $1000$ simulations. Here, we present simulation results for $\mathcal{D}_{\text{sparse}}$ when $P = 10$ covariates and for $\mathcal{D}_{\text{dense}}$ when $P \in \{2,10\}$.

    \begin{table}[H]
        \caption{See the main text.}
    \end{table}

\begin{center}
\renewcommand{\arraystretch}{0.7}
\begin{table}[H]
\caption{Results from 1000 simulated datasets for covariate distribution $\mathcal{D}_{\text{sparse}}$ when $P = 10$ with varying simulation settings and numbers of source sites.}
\label{tab_sparse_10}
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrrrrrrrrrrrr}
  \hline
  & \multicolumn{12}{c}{Simulation scenarios} \\
     \cmidrule(lr){2-13} 
  &  \multicolumn{4}{c}{$K = 10$} &  \multicolumn{4}{c}{$K = 20$} &  \multicolumn{4}{c}{$K = 50$} \\
  %&  \multicolumn{4}{c}{$K = 100$} \\
  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17}
     & Bias & RMSE & Cov. & Len. & Bias & RMSE & Cov. & Len. & Bias & RMSE & Cov. & Len. \\
     %& Bias & RMSE & Cov. & Len. \\
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17}
Specification I &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.01 & 0.76 & 96.00 & 3.22 & 0.00 & 0.71 & 97.60 & 3.24 & 0.00 & 0.76 & 97.30 & 3.25\\
% \hspace{.15cm} SS (naive) & 0.87 & 0.88 & 27.20 & 1.46 & 0.90 & 0.91 & 2.40 & 0.87 & 0.92 & 0.92 & 0.00 & 0.46\\
% \hspace{.15cm} SS     & 0.10 & 0.42 & 99.30 & 2.61 & 0.09 & 0.30 & 99.00 & 1.69 & 0.08 & 0.21 & 96.60 & 0.97\\
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.36 & 0.51 & 96.40 & 2.26 & 0.41 & 0.52 & 87.00 & 1.56 & 0.44 & 0.50 & 54.00 & 0.90\\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.16 & 0.55 & 96.10 & 2.17 & 0.18 & 0.51 & 93.20 & 1.78 & 0.14 & 0.55 & 81.90 & 1.50\\
\hspace{.15cm} Target-Only & 0.01 & 0.76 & 96.00 & 3.22 & 0.00 & 0.71 & 97.60 & 3.24 & 0.00 & 0.76 & 97.30 & 3.25 \\ 
\hspace{.15cm} SS (naive) & 0.87 & 0.88 & 27.20 & 1.46 & 0.90 & 0.91 & 2.40 & 0.87 & 0.92 & 0.92 & 0.00 & 0.46 \\ 
\hspace{.15cm} SS & 0.10 & 0.42 & 99.30 & 2.61 & 0.09 & 0.30 & 99.00 & 1.69 & 0.08 & 0.21 & 96.60 & 0.97 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$ & 0.36 & 0.51 & 96.40 & 2.26 & 0.41 & 0.52 & 87.00 & 1.56 & 0.44 & 0.50 & 54.00 & 0.90 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$ & 0.16 & 0.55 & 96.10 & 2.17 & 0.18 & 0.51 & 93.20 & 1.78 & 0.14 & 0.55 & 81.90 & 1.50 \\ 
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17}
Specification II &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.01 & 0.82 & 95.90 & 3.32 & 0.01 & 0.74 & 97.40 & 3.31 & 0.00 & 0.79 & 97.20 & 3.33 \\
% \hspace{.15cm} SS (naive) & 0.87 & 0.88 & 28.60 & 1.52 & 0.90 & 0.91 & 2.60 & 0.89 & 0.92 & 0.92 & 0.00 & 0.48\\
% \hspace{.15cm} SS     & 0.10 & 0.42 & 99.30 & 2.68 & 0.09 & 0.31 & 99.30 & 1.71 & 0.08 & 0.21 & 97.00 & 0.99\\
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.37 & 0.52 & 96.60 & 2.36 & 0.43 & 0.53 & 87.60 & 1.61 & 0.46 & 0.51 & 54.00 & 0.92\\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.16 & 0.57 & 95.00 & 2.25 & 0.19 & 0.52 & 93.50 & 1.80 & 0.13 & 0.59 & 80.60 & 1.56\\
\hspace{.15cm} Target-Only & 0.01 & 0.82 & 95.90 & 3.32 & 0.01 & 0.74 & 97.40 & 3.31 & 0.00 & 0.79 & 97.20 & 3.33 \\ 
\hspace{.15cm} SS (naive) & 0.87 & 0.88 & 28.60 & 1.52 & 0.90 & 0.91 & 2.60 & 0.89 & 0.92 & 0.92 & 0.00 & 0.48 \\ 
\hspace{.15cm} SS  & 0.10 & 0.42 & 99.30 & 2.68 & 0.09 & 0.31 & 99.30 & 1.71 & 0.08 & 0.21 & 97.00 & 0.99 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$ & 0.37 & 0.52 & 96.60 & 2.36 & 0.43 & 0.53 & 87.60 & 1.61 & 0.46 & 0.51 & 54.00 & 0.92 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$ & 0.16 & 0.57 & 95.00 & 2.25 & 0.19 & 0.52 & 93.50 & 1.80 & 0.13 & 0.59 & 80.60 & 1.56 \\  
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17} 
Specification III &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.04 & 0.76 & 95.60 & 3.24 & 0.06 & 0.74 & 96.40 & 3.24 & 0.06 & 0.79 & 96.70 & 3.29\\
% \hspace{.15cm} SS  (naive)   & 0.84 & 0.86 & 30.80 & 1.52 & 0.87 & 0.88 & 3.70 & 0.92 & 0.89 & 0.89 & 0.00 & 0.49\\
% \hspace{.15cm} SS     & 0.07 & 0.44 & 99.20 & 2.81 & 0.07 & 0.32 & 99.70 & 1.84 & 0.06 & 0.22 & 97.40 & 1.06
% \\
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.31 & 0.48 & 97.00 & 2.27 & 0.37 & 0.48 & 91.00 & 1.60 & 0.40 & 0.47 & 62.80 & 0.92\\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.10 & 0.55 & 96.10 & 2.22 & 0.13 & 0.49 & 94.40 & 1.81 & 0.09 & 0.56 & 82.90 & 1.52\\
\hspace{.15cm} Target-Only & 0.04 & 0.76 & 95.60 & 3.24 & 0.06 & 0.74 & 96.40 & 3.24 & 0.06 & 0.79 & 96.70 & 3.29 \\ 
\hspace{.15cm} SS  (naive)  & 0.84 & 0.86 & 30.80 & 1.52 & 0.87 & 0.88 & 3.70 & 0.92 & 0.89 & 0.89 & 0.00 & 0.49 \\ 
\hspace{.15cm} SS & 0.07 & 0.44 & 99.20 & 2.81 & 0.07 & 0.32 & 99.70 & 1.84 & 0.06 & 0.22 & 97.40 & 1.06 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$ & 0.31 & 0.48 & 97.00 & 2.27 & 0.37 & 0.48 & 91.00 & 1.60 & 0.40 & 0.47 & 62.80 & 0.92 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$ & 0.10 & 0.55 & 96.10 & 2.22 & 0.13 & 0.49 & 94.40 & 1.81 & 0.09 & 0.56 & 82.90 & 1.52 \\ 
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17} 
Specification IV &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.10 & 0.83 & 95.30 & 3.33 & 0.12 & 0.78 & 96.10 & 3.30 & 0.12 & 0.84 & 95.90 & 3.38 \\ 
% \hspace{.15cm} SS  (naive)   & 0.81 & 0.83 & 38.80 & 1.63 & 0.85 & 0.86 & 5.60 & 0.96 & 0.86 & 0.87 & 0.20 & 0.51 \\ 
% \hspace{.15cm} SS     & 0.05 & 0.44 & 99.70 & 2.89 & 0.04 & 0.32 & 99.90 & 1.87 & 0.03 & 0.21 & 98.30 & 1.06 \\ 
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.29 & 0.48 & 97.70 & 2.42 & 0.36 & 0.48 & 92.30 & 1.68 & 0.39 & 0.46 & 64.50 & 0.96 \\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.07 & 0.56 & 95.70 & 2.31 & 0.09 & 0.50 & 93.60 & 1.85 & 0.06 & 0.58 & 82.00 & 1.54 \\
\hspace{.15cm} Target-Only & 0.10 & 0.83 & 95.30 & 3.33 & 0.12 & 0.78 & 96.10 & 3.30 & 0.12 & 0.84 & 95.90 & 3.38 \\ 
\hspace{.15cm} SS  (naive)   & 0.81 & 0.83 & 38.80 & 1.63 & 0.85 & 0.86 & 5.60 & 0.96 & 0.86 & 0.87 & 0.20 & 0.51 \\ 
\hspace{.15cm} SS & 0.05 & 0.44 & 99.70 & 2.89 & 0.04 & 0.32 & 99.90 & 1.87 & 0.03 & 0.21 & 98.30 & 1.06 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$ & 0.29 & 0.48 & 97.70 & 2.42 & 0.36 & 0.48 & 92.30 & 1.68 & 0.39 & 0.46 & 64.50 & 0.96 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$  & 0.07 & 0.56 & 95.70 & 2.31 & 0.09 & 0.50 & 93.60 & 1.85 & 0.06 & 0.58 & 82.00 & 1.54 \\ 
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17}
Specification V &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.01 & 0.82 & 95.90 & 3.32 & 0.01 & 0.74 & 97.40 & 3.31 & 0.00 & 0.79 & 97.10 & 3.33\\
% \hspace{.15cm} SS (naive) & 0.84 & 0.86 & 30.60 & 1.53 & 0.87 & 0.88 & 3.40 & 0.90 & 0.89 & 0.89 & 0.00 & 0.49\\
% \hspace{.15cm} SS     & 0.08 & 0.44 & 99.50 & 2.88 & 0.06 & 0.32 & 99.60 & 1.85 & 0.06 & 0.22 & 97.70 & 1.05\\
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.34 & 0.50 & 96.70 & 2.33 & 0.40 & 0.50 & 89.10 & 1.60 & 0.43 & 0.49 & 57.70 & 0.92\\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.14 & 0.56 & 95.40 & 2.27 & 0.16 & 0.53 & 93.10 & 1.81 & 0.14 & 0.59 & 81.10 & 1.52\\
\hspace{.15cm} Target-Only & 0.01 & 0.82 & 95.90 & 3.32 & 0.01 & 0.74 & 97.40 & 3.31 & 0.00 & 0.79 & 97.10 & 3.33 \\ 
\hspace{.15cm} SS (naive) & 0.84 & 0.86 & 30.60 & 1.53 & 0.87 & 0.88 & 3.40 & 0.90 & 0.89 & 0.89 & 0.00 & 0.49 \\  
\hspace{.15cm} SS  & 0.08 & 0.44 & 99.50 & 2.88 & 0.06 & 0.32 & 99.60 & 1.85 & 0.06 & 0.22 & 97.70 & 1.05 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$  & 0.34 & 0.50 & 96.70 & 2.33 & 0.40 & 0.50 & 89.10 & 1.60 & 0.43 & 0.49 & 57.70 & 0.92 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$ & 0.14 & 0.56 & 95.40 & 2.27 & 0.16 & 0.53 & 93.10 & 1.81 & 0.14 & 0.59 & 81.10 & 1.52 \\ 
\hline
\end{tabular}
Abbreviations: RMSE = Root mean square error; Cov. = Coverage, Len. = Length of $95\%$ CI; \\ SS = Sample Size.
\vspace{.25cm}
\footnotesize{
\begin{flushleft}
\end{flushleft}
}
\end{table}
\end{center}

\begin{center}
\renewcommand{\arraystretch}{0.7}
\begin{table}[H]
\caption{Results from 1000 simulated datasets for covariate distribution $\mathcal{D}_{\text{dense}}$ when $P = 2$ with varying simulation settings and numbers of source sites.}
\label{tab_dense_2}
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrrrrrrrrrrrr}
  \hline
  & \multicolumn{12}{c}{Simulation scenarios} \\
     \cmidrule(lr){2-13} 
  &  \multicolumn{4}{c}{$K = 10$} &  \multicolumn{4}{c}{$K = 20$} &  \multicolumn{4}{c}{$K = 50$} \\
  %&  \multicolumn{4}{c}{$K = 100$} \\
  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17}
     & Bias & RMSE & Cov. & Len. & Bias & RMSE & Cov. & Len. & Bias & RMSE & Cov. & Len. \\
     %& Bias & RMSE & Cov. & Len. \\
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17}
Specification I &  &  &\\ 
%$n_k = 100$ &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.00 & 0.69 & 98.20 & 3.10 & 0.00 & 0.69 & 98.20 & 3.10 & 0.00 & 0.69 & 98.10 & 3.10 \\
% %& 0.02 & 0.64 & 99.00 & 3.07 \\
% \hspace{.15cm} SS (naive) & 0.35 & 0.39 & 91.50 & 1.31 & 0.28 & 0.31 & 75.60 & 0.77 & 0.27 & 0.28 & 22.90 & 0.42 \\
% % & 0.25 & 0.26 & 1.30 & 0.27 \\ 
% \hspace{.15cm} SS     & 0.00 & 0.44 & 99.80 & 2.60 & 0.00 & 0.31 & 98.90 & 1.53 & 0.01 & 0.21 & 95.50 & 0.88 \\
% %& 0.01 & 0.18 & 86.00 & 0.58\\ 
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.08 & 0.26 & 98.60 & 1.42 & 0.06 & 0.20 & 95.10 & 0.86 & 0.07 & 0.17 & 87.30 & 0.50 \\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.04 & 0.41 & 97.30 & 1.68 & 0.03 & 0.38 & 94.80 & 1.30 & 0.03 & 0.44 & 82.00 & 1.15\\
% \hspace{.15cm} $\text{global}-\ell_1$* & 0.04 & 0.39 & 98.00 & 1.63 & 0.03 & 0.31 & 96.20 & 1.18 & 0.03 & 0.26 & 91.70 & 0.88\\
\hspace{.15cm} Target-Only & 0.00 & 0.69 & 98.10 & 3.10 & 0.00 & 0.69 & 98.20 & 3.10 & 0.00 & 0.69 & 98.20 & 3.10 \\ 
\hspace{.15cm} SS (naive) & 0.35 & 0.39 & 91.50 & 1.31 & 0.28 & 0.31 & 75.60 & 0.77 & 0.27 & 0.28 & 22.80 & 0.42\\
\hspace{.15cm} SS & 0.00 & 0.44 & 99.80 & 2.60 & 0.00 & 0.31 & 98.90 & 1.53  & 0.01 & 0.21 & 95.50 & 0.88 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$  & 0.08 & 0.26 & 98.60 & 1.43 & 0.06 & 0.20 & 95.10 & 0.86  & 0.07 & 0.17 & 87.30 & 0.50 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$ & 0.04 & 0.39 & 98.00 & 1.63 & 0.03 & 0.31 & 96.20 & 1.18 & 0.03 & 0.26 & 91.70 & 0.88  \\ 
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17}
Specification II &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.01 & 1.10 & 96.60 & 4.35 & 0.01 & 1.10 & 96.60 & 4.35 & 0.00 & 1.10 & 96.60 & 4.35 \\
% %& 0.03 & 0.95 & 98.00 & 4.14\\
% \hspace{.15cm} SS (naive) & 0.36 & 0.42 & 96.40 & 1.98 & 0.29 & 0.33 & 91.20 & 1.18 & 0.27 & 0.29 & 58.60 & 0.63 \\
% %& 0.26 & 0.27 & 21.60 & 0.41\\
% \hspace{.15cm} SS     & 0.00 & 0.53 & 99.90 & 3.79 & 0.00 & 0.37 & 99.60 & 2.21 & 0.01 & 0.25 & 97.70 & 1.23 \\
% %& 0.03 & 0.20 & 93.00 & 0.81\\ 
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.08 & 0.34 & 99.40 & 2.31 & 0.07 & 0.24 & 98.80 & 1.36 & 0.07 & 0.18 & 95.20 & 0.76 \\
% %& 0.06 & 0.13 & 90.00 & 0.48\\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.04 & 0.54 & 98.50 & 2.29 & 0.04 & 0.48 & 94.30 & 1.65 & 0.03 & 0.60 & 72.40 & 1.34\\
% \hspace{.15cm} $\text{global}-\ell_1$* & 0.04 & 0.40 & 97.90 & 1.67 & 0.04 & 0.31 & 96.40 & 1.19 & 0.04 & 0.26 & 92.60 & 0.88\\
\hspace{.15cm} Target-Only & 0.00 & 0.72 & 97.50 & 3.18 & 0.00 & 0.72 & 97.60 & 3.18 & 0.00 & 0.72 & 97.60 & 3.18\\ 
\hspace{.15cm} SS (naive) & 0.35 & 0.39 & 92.00 & 1.35 & 0.28 & 0.31 & 77.60 & 0.79 & 0.27 & 0.28 & 24.90 & 0.43 \\ 
\hspace{.15cm} SS  & 0.00 & 0.45 & 99.80 & 2.65 & 0.00 & 0.31 & 98.80 & 1.56 & 0.01 & 0.21 & 95.40 & 0.90 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$ & 0.08 & 0.27 & 98.60 & 1.48 & 0.07 & 0.21 & 95.30 & 0.89 & 0.07 & 0.16 & 88.50 & 0.52 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$ & 0.04 & 0.40 & 97.90 & 1.67 & 0.04 & 0.31 & 96.40 & 1.19  & 0.04 & 0.26 & 92.60 & 0.88 \\ 
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17} 
Specification III &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.04 & 0.70 & 96.60 & 3.09 & 0.04 & 0.70 & 96.60 & 3.09 & 0.04 & 0.71 & 96.50 & 3.09 \\
% %& 0.02 & 0.66 & 99.00 & 3.09\\
% \hspace{.15cm} SS (naive) & 0.32 & 0.36 & 94.80 & 1.34 & 0.25 & 0.27 & 85.00 & 0.79 & 0.23 & 0.24 & 40.10 & 0.43 \\
% %& 0.22 & 0.22 & 5.80 & 0.27\\
% \hspace{.15cm} SS     & 0.03 & 0.46 & 99.80 & 2.68 & 0.03 & 0.31 & 99.10 & 1.57 & 0.03 & 0.21 & 96.10 & 0.90 \\
% %& 0.02 & 0.18 & 89.00 & 0.59\\  
% \hspace{.15cm} $\text{global}-\ell_2$  & 0.04 & 0.25 & 99.10 & 1.44 & 0.02 & 0.20 & 95.80 & 0.87 & 0.02 & 0.15 & 90.00 & 0.51 \\
% %& 0.01 & 0.13 & 79.00 & 0.33\\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.00 & 0.41 & 97.20 & 1.67 & 0.01 & 0.39 & 92.70 & 1.30 & 0.02 & 0.46 & 78.60 & 1.14\\
% \hspace{.15cm} $\text{global}-\ell_1$* & 0.00 & 0.40 & 96.90 & 1.63 & 0.01 & 0.31 & 95.00 & 1.18 & \\
\hspace{.15cm} Target-Only & 0.04 & 0.71 & 96.50 & 3.09 & 0.04 & 0.70 & 96.60 & 3.09 & 0.04 & 0.70 & 96.60 & 3.09\\
\hspace{.15cm} SS (naive) & 0.32 & 0.35 & 94.80 & 1.34 & 0.25 & 0.27 & 85.00 & 0.79 & 0.23 & 0.24 & 40.00 & 0.43\\ 
\hspace{.15cm} SS  & 0.03 & 0.45 & 99.80 & 2.68 & 0.03 & 0.31 & 99.10 & 1.57 & 0.03 & 0.21 & 96.10 & 0.90\\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$  & 0.04 & 0.25 & 99.10 & 1.44 & 0.02 & 0.20 & 95.80 & 0.87 & 0.02 & 0.15 & 90.00 & 0.51 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$ & 0.00 & 0.40 & 96.90 & 1.63 & 0.01 & 0.31 & 95.00 & 1.18 & 0.01 & 0.26 & 91.00 & 0.87\\
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17} 
Specification IV &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.10 & 0.74 & 96.80 & 3.18 & 0.32 & 1.17 & 95.30 & 4.38 & 0.32 & 1.18 & 95.30 & 4.38 \\
% %& 0.26 & 1.21 & 97.00 & 4.61\\
% \hspace{.15cm} SS (naive)& 0.14 & 0.26 & 99.90 & 2.19 & 0.05 & 0.18 & 99.40 & 1.29 & 0.05 & 0.11 & 99.10 & 0.68 \\
% %& 0.03 & 0.08 & 98.80 & 0.43\\ 
% \hspace{.15cm} SS     & 0.18 & 0.58 & 100.00 & 3.94 & 0.20 & 0.43 & 99.50 & 2.29 & 0.18 & 0.32 & 96.30 & 1.27 \\
% %& 0.17 & 0.27 & 89.00 & 0.83 \\
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.15 & 0.37 & 98.70 & 2.43 & 0.16 & 0.29 & 97.30 & 1.41 & 0.16 & 0.23 & 90.30 & 0.78  \\
% %& 0.16 & 0.21 & 76.00 & 0.51\\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.21 & 0.59 & 95.50 & 2.35 & 0.22 & 0.53 & 89.00 & 1.64 & 0.25 & 0.64 & 66.40 & 1.25\\
% \hspace{.15cm} $\text{global}-\ell_1$* & 0.04 & 0.54 & 98.50 & 2.29 & 0.04 & 0.48 & 94.30 & 1.65 & 0.03 & 0.60 & 72.40 & 1.34\\
\hspace{.15cm} Target-Only & 0.10 & 0.74 & 96.80 & 3.18 & 0.10 & 0.74 & 96.80 & 3.18 & 0.10 & 0.74 & 96.80 & 3.18 \\ 
\hspace{.15cm} SS (naive) & 0.28 & 0.33 & 97.30 & 1.41 & 0.21 & 0.24 & 91.70 & 0.82  & 0.19 & 0.21 & 61.00 & 0.44\\ 
\hspace{.15cm} SS & 0.06 & 0.46 & 99.80 & 2.73 & 0.06 & 0.32 & 99.20 & 1.60 & 0.06 & 0.22 & 95.90 & 0.92 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$ & 0.01 & 0.26 & 99.30 & 1.50 & 0.02 & 0.20 & 96.70 & 0.90 & 0.02 & 0.15 & 90.40 & 0.52 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$  & 0.04 & 0.41 & 97.10 & 1.67 & 0.05 & 0.31 & 94.50 & 1.18 & 0.05 & 0.26 & 88.50 & 0.86 \\ 
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17}
Specification V &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.01 & 1.10 & 96.60 & 4.35 & 0.01 & 1.10 & 96.60 & 4.35 & 0.00 & 1.10 & 96.60 & 4.35 \\
% %& 0.03 & 0.95 & 98.00 & 4.14\\
% \hspace{.15cm} SS (naive) & 0.30 & 0.37 & 98.20 & 1.96 & 0.24 & 0.29 & 95.40 & 1.18 & 0.21 & 0.24 & 79.00 & 0.63 \\
% %& 0.20 & 0.22 & 44.30 & 0.41\\
% \hspace{.15cm} SS     & 0.01 & 0.54 & 99.90 & 3.84 & 0.01 & 0.37 & 99.70 & 2.24 & 0.01 & 0.25 & 98.10 & 1.25 \\
% %&  0.01 & 0.19 & 98.00 & 0.80\\
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.05 & 0.34 & 99.40 & 2.29 & 0.05 & 0.24 & 99.00 & 1.35 & 0.04 & 0.17 & 96.00 & 0.75 \\
% %& 0.03 & 0.12 & 93.00 & 0.47\\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.03 & 0.53 & 98.10 & 2.27 & 0.03 & 0.47 & 93.60 & 1.62 & 0.02 & 0.61 & 71.40 & 1.31\\
\hspace{.15cm} Target-Only & 0.00 & 0.72 & 97.50 & 3.18 & 0.00 & 0.72 & 97.60 & 3.18 & 0.00 & 0.72 & 97.60 & 3.18 \\ 
\hspace{.15cm} SS (naive) & 0.33 & 0.37 & 93.90 & 1.35 & 0.27 & 0.29 & 81.90 & 0.79 & 0.25 & 0.26 & 32.60 & 0.43 \\ 
\hspace{.15cm} SS & 0.01 & 0.45 & 99.80 & 2.71 & 0.00 & 0.31 & 98.80 & 1.59 & 0.00 & 0.21 & 95.90 & 0.92  \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$ & 0.07 & 0.26 & 98.70 & 1.47 & 0.06 & 0.20 & 95.80 & 0.89  & 0.06 & 0.16 & 89.60 & 0.52 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$ & 0.04 & 0.39 & 98.20 & 1.65 & 0.03 & 0.31 & 96.30 & 1.18 & 0.03 & 0.25 & 92.80 & 0.87\\
\hline
\end{tabular}
Abbreviations: RMSE = Root mean square error; Cov. = Coverage, Len. = Length of $95\%$ CI; \\ SS = Sample Size.
\vspace{.25cm}
\footnotesize{
\begin{flushleft}
\end{flushleft}
}
\end{table}
\end{center}

\begin{center}
\renewcommand{\arraystretch}{0.7}
\begin{table}[H]
% \caption{The absolute bias, root mean squared error, coverage and length of the 95\% confidence interval in 1000 simulation datasets for covariates distribution $\mathcal{D}_{\text{dense}}$ when $P = 10$.}
\caption{Results from 1000 simulated datasets for covariate distribution $\mathcal{D}_{\text{dense}}$ when $P = 10$ with varying simulation settings and numbers of source sites.}
\label{tab_dense_10}
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrrrrrrrrrrrr}
  \hline
  & \multicolumn{12}{c}{Simulation scenarios} \\
     \cmidrule(lr){2-13} 
  &  \multicolumn{4}{c}{$K = 10$} &  \multicolumn{4}{c}{$K = 20$} &  \multicolumn{4}{c}{$K = 50$} \\
  %&  \multicolumn{4}{c}{$K = 100$} \\
  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17}
     & Bias & RMSE & Cov. & Len. & Bias & RMSE & Cov. & Len. & Bias & RMSE & Cov. & Len. \\
     %& Bias & RMSE & Cov. & Len. \\
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17}
Specification I &  &  &\\ 
%$n_k = 100$ &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.13 & 2.63 & 95.30 & 7.46 & 0.13 & 2.63 & 95.30 & 7.46 & 0.13 & 2.63 & 95.30 & 7.46\\
% %& 0.05 & 1.67 & 97.00 & 6.53 \\
% %& 0.09 & 1.66 & 97.00 & 6.51\\
% \hspace{.15cm} SS (naive) & 0.22 & 0.46 & 99.50 & 5.09 & 0.19 & 0.33 & 99.00 & 2.89 & 0.18 & 0.25 & 94.90 & 1.40\\
% %& 0.18 & 0.21 & 86.30 & 0.84\\ 
% \hspace{.15cm} SS     & 0.00 & 0.70 & 100.00 & 7.65 & 0.01 & 0.47 & 99.80 & 4.27 & 0.01 & 0.31 & 99.70 & 2.19\\ %& 0.00 & 0.20 & 100.00 & 1.17\\
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.06 & 0.53 & 99.80 & 6.31 & 0.07 & 0.38 & 99.40 & 3.45 & 0.07 & 0.25 & 98.40 & 1.71\\
% %& 0.07 & 0.18 & 98.00 & 0.85\\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.01 & 0.90 & 97.80 & 5.79 & 0.02 & 0.80 & 92.50 & 3.56 & 0.02 & 0.96 & 65.10 & 2.35\\
\hspace{.15cm} Target-Only & 0.13 & 2.63 & 95.30 & 7.46 & 0.13 & 2.63 & 95.30 & 7.46 & 0.13 & 2.63 & 95.30 & 7.46 \\  
\hspace{.15cm} SS (naive) & 0.22 & 0.46 & 99.50 & 5.09 & 0.19 & 0.33 & 99.00 & 2.89 & 0.18 & 0.25 & 94.90 & 1.40 \\ 
\hspace{.15cm} SS & 0.00 & 0.70 & 100.00 & 7.65 & 0.01 & 0.47 & 99.80 & 4.27 & 0.01 & 0.31 & 99.70 & 2.19 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$ & 0.06 & 0.53 & 99.80 & 6.31 & 0.07 & 0.38 & 99.40 & 3.45 & 0.07 & 0.25 & 98.40 & 1.71 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$ & 0.01 & 0.80 & 98.40 & 5.76 & 0.04 & 0.57 & 97.60 & 3.42 & 0.06 & 0.40 & 95.90 & 1.83 \\ 
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17}
Specification II &  &  &\\ 
% \hspace{.15cm} target & 0.02 & 3.38 & 93.90 & 10.21 & 0.02 & 3.38 & 93.90 & 10.21 & 0.02 & 3.39 & 93.90 & 10.21 \\
% %& 0.07 & 2.47 & 96.00 & 8.95\\
% \hspace{.15cm} ss (naive) & 0.22 & 0.61 & 99.90 & 8.24 & 0.19 & 0.45 & 99.50 & 4.65 & 0.19 & 0.31 & 98.60 & 2.22\\
% %& 0.18 & 0.25 & 94.60 & 1.33\\
% \hspace{.15cm} ss     & 0.00 & 1.03 & 99.90 & 12.80 & 0.01 & 0.69 & 100.00 & 6.97 & 0.01 & 0.42 & 99.90 & 3.38 \\
% %& 0.02 & 0.28 & 100.00 & 1.83\\  
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.11 & 0.75 & 100.00 & 10.32 & 0.11 & 0.53 & 99.70 & 5.52 & 0.12 & 0.35 & 99.30 & 2.67\\
% %& 0.10 & 0.27 & 98.00 & 1.34\\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.10 & 1.24 & 97.90 & 8.71 & 0.10 & 1.12 & 94.00 & 5.32 & 0.09 & 1.39 & 65.80 & 3.33 \\
\hspace{.15cm} Target-Only & 0.10 & 2.50 & 95.40 & 7.55 & 0.10 & 2.50 & 95.40 & 7.55 & 0.10 & 2.50 & 95.40 & 7.55 \\ 
\hspace{.15cm} SS (naive) & 0.22 & 0.46 & 99.40 & 4.89 & 0.19 & 0.34 & 99.20 & 2.78 & 0.18 & 0.25 & 95.70 & 1.36 \\ 
\hspace{.15cm} SS & 0.00 & 0.72 & 100.00 & 7.52 & 0.01 & 0.48 & 99.80 & 4.19 & 0.01 & 0.31 & 99.60 & 2.17 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$ & 0.07 & 0.54 & 99.90 & 6.14 & 0.08 & 0.38 & 99.40 & 3.36 & 0.08 & 0.25 & 98.60 & 1.69 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$ & 0.04 & 0.82 & 98.10 & 5.53 & 0.06 & 0.57 & 97.40 & 3.30 & 0.07 & 0.41 & 96.50 & 1.79 \\ 
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17} 
Specification III &  &  &\\ 
% \hspace{.15cm} target & 0.12 & 2.06 & 93.20 & 7.08 & 0.12 & 2.06 & 93.20 & 7.08 & 0.12 & 2.06 & 93.20 & 7.08 \\
% %& 0.13 & 1.95 & 93.00 & 6.50\\
% \hspace{.15cm} ss  (naive)   & 0.19 & 0.46 & 99.70 & 4.12 & 0.17 & 0.33 & 99.00 & 2.41 & 0.16 & 0.25 & 95.30 & 1.23 \\
% %& 0.16 & 0.21 & 89.60 & 0.76\\
% \hspace{.15cm} ss     & 0.03 & 0.87 & 100.00 & 8.11 & 0.01 & 0.59 & 100.00 & 4.63 & 0.02 & 0.38 & 99.90 & 2.42
% \\
% %& 0.04 & 0.28 & 100.00 & 1.43\\ 
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.02 & 0.53 & 99.40 & 5.23 & 0.04 & 0.37 & 99.60 & 2.92 & 0.04 & 0.24 & 98.80 & 1.51 \\
% %& 0.02 & 0.17 & 99.00 & 0.91\\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.02 & 0.90 & 97.10 & 4.54 & 0.01 & 0.83 & 93.20 & 2.97& 0.04 & 0.99 & 65.90 & 2.12\\
\hspace{.15cm} Target-Only & 0.12 & 2.06 & 93.20 & 7.08 & 0.12 & 2.06 & 93.20 & 7.08 & 0.12 & 2.06 & 93.20 & 7.08 \\ 
\hspace{.15cm} SS (naive) & 0.19 & 0.46 & 99.70 & 4.12 & 0.17 & 0.33 & 99.00 & 2.41 & 0.16 & 0.25 & 95.30 & 1.23 \\ 
\hspace{.15cm} SS & 0.03 & 0.87 & 100.00 & 8.11 & 0.01 & 0.59 & 100.00 & 4.63 & 0.02 & 0.38 & 99.90 & 2.42 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$ & 0.02 & 0.53 & 99.40 & 5.23 & 0.04 & 0.37 & 99.60 & 2.92 & 0.04 & 0.24 & 98.80 & 1.51 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$ & 0.01 & 0.84 & 97.70 & 4.52 & 0.01 & 0.60 & 97.50 & 2.82 & 0.03 & 0.38 & 96.30 & 1.57 \\ 
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17} 
Specification IV &  &  &\\ 
% \hspace{.15cm} target & 0.59 & 2.92 & 92.30 & 9.90 & 0.59 & 2.92 & 92.30 & 9.90 & 0.58 & 2.92 & 92.30 & 9.91\\
% %& 0.81 & 2.83 & 87.88 & 9.15\\
% \hspace{.15cm} ss (naive)  & 0.34 & 0.70 & 99.50 & 7.18 & 0.38 & 0.57 & 98.70 & 4.19 & 0.37 & 0.47 & 94.50 & 2.10\\
% %& 0.37 & 0.42 & 80.00 & 1.28\\ 
% \hspace{.15cm} ss     & 0.57 & 1.36 & 99.80 & 14.04 & 0.57 & 1.03 & 99.70 & 7.93 & 0.54 & 0.77 & 98.20 & 3.90\\
% %& 0.51 & 0.64 & 87.00 & 2.32\\ 
% \hspace{.15cm} $\text{global}-\ell_2$  & 0.49 & 0.91 & 99.20 & 9.19 & 0.47 & 0.71 & 98.20 & 4.92 & 0.45 & 0.57 & 94.00 & 2.44\\
% %& 0.48 & 0.54 & 76.77 & 1.43\\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.50 & 1.42 & 95.10 & 7.18 & 0.52 & 1.32 & 88.20 & 4.62 & 0.53 & 1.56 & 64.60 & 3.56 \\
\hspace{.15cm} Target-Only & 0.21 & 2.01 & 92.90 & 7.16 & 0.21 & 2.01 & 92.90 & 7.16 & 0.21 & 2.01 & 92.90 & 7.16 \\ 
\hspace{.15cm} SS (naive)  & 0.08 & 0.44 & 99.70 & 4.09 & 0.06 & 0.30 & 99.70 & 2.40 & 0.06 & 0.20 & 98.40 & 1.23 \\ 
\hspace{.15cm} SS  & 0.14 & 0.89 & 100.00 & 8.12 & 0.13 & 0.62 & 99.90 & 4.70 & 0.12 & 0.41 & 99.70 & 2.44 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$ & 0.09 & 0.55 & 99.30 & 5.25 & 0.07 & 0.38 & 99.20 & 2.92 & 0.06 & 0.25 & 99.10 & 1.51 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$ & 0.11 & 0.86 & 97.40 & 4.44 & 0.10 & 0.62 & 96.60 & 2.80 & 0.07 & 0.41 & 95.10 & 1.57 \\ 
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17}
Specification V &  &  &\\ 
% \hspace{.15cm} target & 0.02 & 3.38 & 93.90 & 10.21 & 0.02 & 3.38 & 93.90 & 10.21  & 0.02 & 3.39 & 93.90 & 10.21\\
% %& 0.07 & 2.47 & 96.00 & 8.95\\
% \hspace{.15cm} SS (naive) & 0.04 & 0.59 & 99.80 & 8.33 & 0.05 & 0.42 & 99.90 & 4.74 & 0.05 & 0.42 & 99.90 & 4.74 \\
% %& 0.07 & 0.20 & 98.80 & 1.38 \\
% \hspace{.15cm} SS    & 0.29 & 1.28 & 99.90 & 15.48 & 0.25 & 0.89 & 100.00 & 8.57 & 0.25 & 0.59 & 99.80 & 4.12 \\
% %& 0.20 & 0.45 & 98.00 & 2.25\\  
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.11 & 0.77 & 100.00 & 10.37 & 0.08 & 0.53 & 99.70 & 5.52 & 0.10 & 0.35 & 99.10 & 2.68 \\
% %& 0.10 & 0.28 & 97.00 & 1.35\\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.02 & 1.30 & 97.00 & 8.68 & 0.04 & 1.15 & 94.00 & 5.33 & 0.01 & 1.39 & 66.60 & 3.33\\
\hspace{.15cm} Target-Only & 0.10 & 2.50 & 95.40 & 7.55 & 0.10 & 2.50 & 95.40 & 7.55 & 0.10 & 2.50 & 95.40 & 7.55 \\ 
\hspace{.15cm} SS (naive) & 0.15 & 0.45 & 99.80 & 4.97 & 0.13 & 0.32 & 99.30 & 2.84 & 0.12 & 0.22 & 97.70 & 1.40 \\ 
\hspace{.15cm} SS  & 0.07 & 0.89 & 100.00 & 9.00 & 0.05 & 0.61 & 99.90 & 5.14 & 0.05 & 0.39 & 99.80 & 2.60 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$ & 0.01 & 0.55 & 99.80 & 6.14 & 0.03 & 0.37 & 99.60 & 3.36 & 0.02 & 0.24 & 98.40 & 1.69 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$  & 0.00 & 0.82 & 98.50 & 5.52 & 0.00 & 0.57 & 97.70 & 3.31 & 0.03 & 0.41 & 96.10 & 1.81 \\ 
\hline
\end{tabular}
Abbreviations: RMSE = Root mean square error; Cov. = Coverage, Len. = Length of $95\%$ CI; \\ SS = Sample Size.
\vspace{.25cm}
\footnotesize{
\begin{flushleft}
\end{flushleft}
}
\end{table}
\end{center}

\begin{center}
\renewcommand{\arraystretch}{0.7}
\begin{table}[H]
\caption{Results from 500 simulated datasets when $P = 2$ anchoring total population with varying simulation settings and numbers of source sites. The true effects are uniform across all the sites in Setting $\text{GATE}_{\text{uniform}}$ and vary in Setting $\text{GATE}_{\text{various}}$.}
\label{tab_wave2_2}
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrrrrrrrrrrrr}
  \hline
  & \multicolumn{12}{c}{Simulation scenarios} \\
     \cmidrule(lr){2-13} 
  &  \multicolumn{4}{c}{$K = 10$} &  \multicolumn{4}{c}{$K = 20$} &  \multicolumn{4}{c}{$K = 50$} \\
  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
     $\text{GATE}_{\text{uniform}}$ & Bias & RMSE & Cov. & Len. & Bias & RMSE & Cov. & Len. & Bias & RMSE & Cov. & Len. \\
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
Specification I &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.02 & 0.63 & 100.00 & 3.07 & 0.02 & 0.63 & 100.00 & 3.08 & 0.02 & 0.62 & 100.00 & 3.08 \\
% \hspace{.15cm} ss (naive) & 0.02 & 0.15 & 99.00 & 0.94 & 0.03 & 0.12 & 98.00 & 0.60 & 0.03 & 0.07 & 98.00 & 0.35\\
% \hspace{.15cm} ss & 0.02  & 0.15 & 99.00 & 0.93 & 0.03 & 0.12 & 98.00 & 0.60 & 0.02 & 0.07 & 98.00 & 0.35 \\
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.01 & 0.17 & 100.00 & 1.03 & 0.00 & 0.13 & 100.00 & 0.66 & 0.02 & 0.09 & 98.00 & 0.39 \\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.02 & 0.23 & 99.00 & 1.28 & 0.01 & 0.20 & 100.00 & 0.96 & 0.02 & 0.16 & 100.00 & 0.73\\
% \hspace{.15cm} Fixed-effects & 0.03 & 0.57 & 98.00 & 2.42 & 0.03 & 0.57 & 96.00 & 2.42 & 0.03 & 0.57 & 95.00 & 2.41\\
\hspace{.15cm} Target-Only & 0.02 & 0.69 & 98.00 & 3.11 & 0.02 & 0.69 & 98.00 & 3.12 & 0.02 & 0.69 & 98.00 & 3.12 \\ 
\hspace{.15cm} SS (naive) & 0.00 & 0.15 & 99.00 & 0.98 & 0.00 & 0.11 & 99.00 & 0.62 & 0.01 & 0.07 & 98.80 & 0.36 \\ 
\hspace{.15cm} SS & 0.00 & 0.16 & 99.20 & 0.97 & 0.00 & 0.11 & 98.80 & 0.62 & 0.01 & 0.07 & 98.80 & 0.36 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$ & 0.04 & 0.18 & 99.40 & 1.07 & 0.04 & 0.14 & 98.60 & 0.69 & 0.04 & 0.09 & 97.60 & 0.40 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$ & 0.03 & 0.27 & 99.20 & 1.29 & 0.03 & 0.22 & 99.40 & 0.97 & 0.03 & 0.17 & 98.60 & 0.73 \\ 
\hspace{.15cm} Fixed-effects & 0.02 & 0.63 & 95.20 & 2.42 & 0.01 & 0.63 & 95.00 & 2.42 & 0.01 & 0.63 & 94.60 & 2.41 \\ 
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13}
Specification II &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.03 & 0.69 & 97.00 & 3.30 & 0.03 & 0.69 & 97.00 & 3.31 & 0.03 & 0.69 & 97.00 & 3.31 \\
% \hspace{.15cm} ss (naive) &  0.02 & 0.18 & 99.00 & 1.09 & 0.03 & 0.14 & 98.00 & 0.70 & 0.03 & 0.09 & 97.00 & 0.40\\
% \hspace{.15cm} ss & 0.03  & 0.18 & 99.00 & 1.08 & 0.04 & 0.14 & 97.00 & 0.70 & 0.03 & 0.09 & 97.00 & 0.40 \\
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.03 & 0.19 & 100.00 & 1.17 & 0.04 & 0.15 & 100.00 & 0.75 & 0.02 & 0.10 & 95.00 & 0.44 \\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.03 & 0.31 & 98.00 & 1.38 & 0.04 & 0.21 & 97.00 & 0.97 & 0.03 & 0.16 & 97.00 & 0.69\\
% \hspace{.15cm} Fixed-effects & 0.12 & 0.63 & 97.00 & 2.64 & 0.12 & 0.63 & 96.00 & 2.63 & 0.12 & 0.62 & 97.00 & 2.63\\
\hspace{.15cm} Target-Only & 0.04 & 0.83 & 95.40 & 3.43 & 0.04 & 0.84 & 95.40 & 3.44 & 0.04 & 0.84 & 95.40 & 3.44 \\ 
\hspace{.15cm} SS (naive) & 0.00 & 0.18 & 99.00 & 1.18 & 0.01 & 0.13 & 99.00 & 0.74 & 0.01 & 0.08 & 98.60 & 0.42 \\ 
\hspace{.15cm} SS & 0.01 & 0.18 & 99.00 & 1.19 & 0.01 & 0.13 & 98.80 & 0.75 & 0.02 & 0.08 & 98.20 & 0.42 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$ & 0.00 & 0.20 & 99.00 & 1.26 & 0.01 & 0.15 & 99.00 & 0.80 & 0.01 & 0.09 & 97.60 & 0.46 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$ & 0.01 & 0.28 & 98.60 & 1.41 & 0.02 & 0.22 & 97.80 & 1.01 & 0.02 & 0.17 & 96.40 & 0.70 \\ 
\hspace{.15cm} Fixed-effects & 0.14 & 0.69 & 95.20 & 2.64 & 0.14 & 0.69 & 95.40 & 2.63 & 0.13 & 0.69 & 95.80 & 2.63 \\ 
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
  $\text{GATE}_{\text{various}}$ & Bias & RMSE & Cov. & Len. & Bias & RMSE & Cov. & Len. & Bias & RMSE & Cov. & Len. \\
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
Specification I  &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.02 & 0.63 & 100.00  & 3.07 & 0.02 & 0.63 & 100.00 & 3.08 & 0.02 & 0.62 & 100.00 & 3.08 \\
% \hspace{.15cm} ss (naive) &  0.28 & 0.37 & 96.00 & 1.31 & 0.26 & 0.32 & 79.00 & 0.81 & 0.23 & 0.27 & 46.00 & 0.43 \\
% \hspace{.15cm} ss & 0.28 & 0.37 & 95.00 & 1.30 & 0.26 & 0.32 & 81.00 & 0.80 & 0.23 & 0.27 & 45.00 & 0.43 \\
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.09 & 0.21 & 98.00 & 1.16 & 0.06 & 0.17 & 96.00 & 0.73 & 0.02 & 0.12 & 89.00 & 0.42\\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.08 &  0.28 & 99.00 & 1.39 & 0.05 & 0.23 & 99.00 & 1.06 & 0.02 & 0.19 & 98.00 & 0.81 \\
% \hspace{.15cm} Fixed-effects & 0.03 & 0.57 & 98.00 & 2.42 & 0.03 & 0.57 & 96.00 & 2.42 & 0.03 & 0.57 & 95.00 & 2.41 \\
\hspace{.15cm} Target-Only & 0.02 & 0.69 & 98.00 & 3.11 & 0.02 & 0.69 & 98.00 & 3.12 & 0.02 & 0.69 & 98.00 & 3.12 \\ 
\hspace{.15cm} SS (naive) & 0.32 & 0.42 & 93.20 & 1.38 & 0.28 & 0.35 & 76.00 & 0.82 & 0.25 & 0.28 & 40.20 & 0.44 \\ 
\hspace{.15cm} SS & 0.32 & 0.42 & 93.00 & 1.38 & 0.28 & 0.35 & 75.60 & 0.83 & 0.25 & 0.28 & 40.40 & 0.44 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$ & 0.12 & 0.25 & 97.40 & 1.20 & 0.07 & 0.18 & 94.60 & 0.75 & 0.03 & 0.12 & 92.20 & 0.42 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$ & 0.09 & 0.31 & 99.20 & 1.40 & 0.05 & 0.26 & 98.00 & 1.07 & 0.02 & 0.21 & 95.80 & 0.81 \\ 
\hspace{.15cm} Fixed-effects & 0.02 & 0.63 & 95.20 & 2.42 & 0.01 & 0.63 & 95.00 & 2.42 & 0.01 & 0.63 & 94.60 & 2.41 \\ 
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13}
Specification II &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.03 & 0.69 & 97.00 & 3.30 & 0.03 & 0.69 & 97.00 & 3.31 & 0.03 & 0.69 & 97.00 & 3.31  \\
% \hspace{.15cm} ss (naive) & 0.29 & 0.38 & 97.00 & 1.48 & 0.26 & 0.32 & 87.00 & 0.90 & 0.23 & 0.27 & 59.00 & 0.48 \\
% \hspace{.15cm} ss & 0.28  & 0.38 & 97.00 & 1.46 & 0.25 & 0.32 & 89.00 & 0.90 & 0.23 & 0.27 & 61.00 & 0.48 \\
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.03 & 0.21 & 99.00 & 1.32 & 0.01 & 0.17 & 98.00 & 0.82 & 0.05 & 0.14 & 89.00  & 0.46  \\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.07 & 0.43 & 96.00 & 1.50 &  0.01 & 0.24 & 97.00 & 1.06 & 0.04 & 0.19 & 96.00 & 0.76  \\
% \hspace{.15cm} Fixed-effects & 0.12 & 0.63 & 97.00 & 2.64 & 0.12 & 0.63 & 96.00 & 2.63 & 0.12 & 0.62 & 97.00 & 2.63\\
\hspace{.15cm} Target-Only & 0.04 & 0.83 & 95.40 & 3.43 & 0.04 & 0.84 & 95.40 & 3.44 & 0.04 & 0.84 & 95.40 & 3.44 \\ 
\hspace{.15cm} SS (naive) & 0.32 & 0.43 & 94.80 & 1.60 & 0.28 & 0.35 & 83.00 & 0.95 & 0.24 & 0.28 & 52.80 & 0.50 \\ 
\hspace{.15cm} SS & 0.31 & 0.43 & 95.20 & 1.61 & 0.28 & 0.35 & 83.60 & 0.95 & 0.24 & 0.27 & 56.00 & 0.50 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_2$ & 0.06 & 0.24 & 98.60 & 1.39 & 0.00 & 0.18 & 96.40 & 0.86 & 0.04 & 0.13 & 91.80 & 0.48 \\ 
\hspace{.15cm} $\text{GLOBAL}-\ell_1$ & 0.03 & 0.32 & 98.60 & 1.52 & 0.01 & 0.27 & 96.40 & 1.09 & 0.05 & 0.21 & 93.20 & 0.77 \\ 
\hspace{.15cm} Fixed-effects & 0.14 & 0.69 & 95.20 & 2.64 & 0.14 & 0.69 & 95.40 & 2.63 & 0.13 & 0.69 & 95.80 & 2.63 \\ 
\hline
\end{tabular}
Abbreviations: RMSE = Root mean square error; Cov. = Coverage, Len. = Length of $95\%$ CI.
\vspace{.25cm}
\footnotesize{
\begin{flushleft}
\end{flushleft}
}
\end{table}
\end{center}

\begin{center}
\renewcommand{\arraystretch}{0.7}
\begin{table}[H]
\caption{Results from 500 simulated datasets when $P = 10$ anchoring total population with varying simulation settings and numbers of source sites. The true effects are uniform across all the sites.}
\label{tab_wave2_10}
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrrrrrrrrrrrr}
  \hline
  & \multicolumn{12}{c}{Simulation scenarios} \\
     \cmidrule(lr){2-13} 
  &  \multicolumn{4}{c}{$K = 10$} &  \multicolumn{4}{c}{$K = 20$} &  \multicolumn{4}{c}{$K = 50$} \\
  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
     $\text{GATE}_{\text{uniform}}$ & Bias & RMSE & Cov. & Len. & Bias & RMSE & Cov. & Len. & Bias & RMSE & Cov. & Len. \\
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
Specification I &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.08 & 1.84 & 95.00 & 7.12 & 0.10 & 1.83 & 95.00 & 7.12 & 0.12 & 1.84 & 95.00 & 7.15 \\
% \hspace{.15cm} ss (naive) & 0.03 & 0.40 & 100.00 & 3.24 & 0.01 & 0.25 & 100.00 & 1.96 & 0.02 & 0.15 & 100.00  & 1.03  \\
% \hspace{.15cm} ss & 0.02 & 0.39 & 99.00 & 3.62 & 0.00 & 0.25 & 100.00 & 2.14 & 0.02 & 0.16 & 99.00 & 1.12  \\
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.02 & 0.41 & 99.00 & 3.68 & 0.04 & 0.29 & 100.00 & 2.14 & 0.03 & 0.18 & 100.00 & 1.14 \\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.01 & 0.56 & 99.00 & 3.41 & 0.07 & 0.45 & 98.00 & 2.17 & 0.04 & 0.25 & 98.00 & 1.20\\
% \hspace{.15cm} Fixed-effects & 0.00 & 1.38 & 93.00 & 5.34 & 0.03 & 1.38 & 94.00 & 5.31 & 0.04 & 1.39 & 93.00 & 5.30\\
\hspace{.15cm} Target-Only  & 0.11 & 3.48 & 95.60 & 8.42 & 0.11 & 3.41 & 95.80 & 8.41 & 0.09 & 3.26 & 95.80 & 8.37 \\ 
\hspace{.15cm} SS (naive) & 0.04 & 0.42 & 99.80 & 6.37 & 0.01 & 0.28 & 99.40 & 3.57 & 0.01 & 0.18 & 99.60 & 1.68 \\ 
\hspace{.15cm} SS & 0.04 & 0.43 & 99.60 & 7.16 & 0.02 & 0.28 & 99.20 & 3.90 & 0.01 & 0.18 & 99.40 & 1.73 \\ 
\hspace{.15cm} $\text{global}-\ell_2$ & 0.02 & 0.48 & 99.80 & 7.22 & 0.04 & 0.33 & 99.60 & 3.92 & 0.04 & 0.21 & 98.80 & 1.75 \\ 
\hspace{.15cm} $\text{global}-\ell_1$ & 0.03 & 0.58 & 99.40 & 7.24 & 0.05 & 0.43 & 97.40 & 4.06 & 0.05 & 0.30 & 96.20 & 2.01 \\ 
\hspace{.15cm} Fixed-effects  & 0.05 & 1.36 & 93.20 & 5.33 & 0.03 & 1.36 & 94.00 & 5.31 & 0.03 & 1.36 & 93.60 & 5.30 \\ 
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13}
Specification II  &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.05 & 1.99 & 95.00 & 7.64 & 0.03 & 2.02 & 96.00 & 7.66 & 0.02 & 2.03 & 96.00 & 7.69 \\
% \hspace{.15cm} ss (naive) & 0.03 & 0.43 & 99.00 & 3.71 & 0.02 & 0.28 & 100.00 & 2.28 & 0.03 & 0.17 & 99.00 & 1.20\\
% \hspace{.15cm} ss & 0.06  & 0.43 & 100.00 & 4.13 & 0.04 & 0.28 & 100.00 & 2.50 & 0.05 & 0.18 & 99.00 & 1.30 \\
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.12 & 0.48 & 100.00 & 4.11 & 0.09 & 0.33 & 98.00 & 2.46 & 0.09 & 0.21 & 98.00 & 1.30 \\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.09 & 0.80 & 96.00 & 3.84 & 0.05 & 0.52 & 97.00 & 2.42 & 0.08 & 0.45 & 95.00 & 1.37\\
% \hspace{.15cm} Fixed-effects & 0.27 & 1.46 & 96.00 & 5.87 & 0.24 & 1.48 & 96.00 & 5.84 & 0.24 & 1.49 & 96.00 & 5.83\\
\hspace{.15cm} Target-Only & 0.10 & 3.14 & 93.80 & 8.96 & 0.10 & 3.10 & 93.60 & 8.97 & 0.09 & 3.04 & 94.20 & 8.95 \\ 
\hspace{.15cm} SS (naive) & 0.05 & 0.44 & 99.60 & 6.11 & 0.03 & 0.31 & 99.80 & 3.46 & 0.03 & 0.20 & 98.60 & 1.67 \\ 
\hspace{.15cm} SS & 0.08 & 0.46 & 99.80 & 6.55 & 0.07 & 0.32 & 99.40 & 3.63 & 0.06 & 0.21 & 98.80 & 1.72 \\ 
\hspace{.15cm} $\text{global}-\ell_2$  & 0.10 & 0.51 & 99.80 & 6.59 & 0.09 & 0.37 & 99.00 & 3.64 & 0.09 & 0.24 & 97.60 & 1.72 \\ 
\hspace{.15cm} $\text{global}-\ell_1$  & 0.12 & 0.72 & 98.60 & 6.41 & 0.09 & 0.48 & 98.00 & 3.63 & 0.09 & 0.34 & 96.00 & 1.78 \\ 
\hspace{.15cm} Fixed-effects & 0.28 & 1.50 & 93.80 & 5.87 & 0.26 & 1.50 & 93.40 & 5.84 & 0.26 & 1.50 & 94.00 & 5.83 \\ 
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13}  $\text{GATE}_{\text{various}}$ & Bias & RMSE & Cov. & Len. & Bias & RMSE & Cov. & Len. & Bias & RMSE & Cov. & Len. \\
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
Specification I  &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.08 & 1.84 & 95.00 & 7.12 & 0.10 & 1.83 & 95.00  & 7.12 &  0.12 & 1.84 & 95.00 & 7.15  \\
% \hspace{.15cm} ss (naive) & 0.28 & 0.54 & 99.00 & 3.60 & 0.28 & 0.39 & 98.00 & 2.13 & 0.24 & 0.30 & 93.00 &  1.10   \\
% \hspace{.15cm} ss & 0.28 & 0.54 & 99.00 & 4.02 & 0.29 & 0.39 &  99.00 &  2.31 & 0.24 & 0.31 & 94.00 & 1.18  \\
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.07 & 0.47 & 99.00 & 3.81 & 0.04 & 0.31 & 100.00 & 2.20 & 0.02 & 0.20 & 98.00  & 1.17  \\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.09 & 0.56 & 99.00 & 3.52 & 0.07 & 0.47 & 99.00 & 2.21 & 0.00 & 0.29 & 97.00 & 1.24  \\
% \hspace{.15cm} Fixed-effects & 0.00 & 1.38 & 93.00 & 5.34 & 0.03 & 1.38 & 94.00 & 5.31 & 0.04 & 1.39 & 93.00 &  5.30 \\
\hspace{.15cm} Target-Only & 0.11 & 3.48 & 95.60 & 8.42 & 0.11 & 3.41 & 95.80 & 8.41 & 0.09 & 3.26 & 95.80 & 8.37 \\ 
\hspace{.15cm} Target-Only & 0.29 & 0.57 & 98.80 & 6.79 & 0.28 & 0.42 & 97.40 & 3.82 & 0.25 & 0.32 & 90.60 & 1.76 \\ 
\hspace{.15cm} SS & 0.29 & 0.58 & 99.40 & 7.58 & 0.27 & 0.43 & 97.80 & 4.14 & 0.25 & 0.32 & 92.20 & 1.81 \\ 
\hspace{.15cm} $\text{global}-\ell_2$ & 0.06 & 0.51 & 99.40 & 7.32 & 0.03 & 0.35 & 99.40 & 3.97 & 0.01 & 0.23 & 97.60 & 1.77 \\ 
\hspace{.15cm} $\text{global}-\ell_1$ & 0.08 & 0.64 & 98.80 & 7.38 & 0.03 & 0.49 & 97.80 & 4.04 & 0.00 & 0.32 & 96.60 & 2.00 \\ 
\hspace{.15cm} Fixed-effects & 0.05 & 1.36 & 93.20 & 5.33 & 0.03 & 1.36 & 94.00 & 5.31 & 0.03 & 1.36 & 93.60 & 5.30 \\ 
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17}
Specification II &  &  &\\ 
% \hspace{.15cm} Target-Only & 0.05 & 1.99 & 95.00 & 7.64 & 0.03 & 2.02 & 96.00 &  7.66 & 0.02 & 2.03 & 96.00 & 7.69 \\
% \hspace{.15cm} ss (naive) & 0.27 & 0.56 & 99.00 & 4.10 & 0.27 & 0.40 & 100.00 & 2.46 & 0.23 & 0.31 & 96.00 & 1.27  \\
% \hspace{.15cm} ss & 0.25 & 0.54 & 99.00 & 4.55 & 0.25 & 0.39 & 100.00 & 2.68 & 0.21 & 0.29 & 97.00 & 1.36 \\
% \hspace{.15cm} $\text{global}-\ell_2$   & 0.07 & 0.52 & 99.00 & 4.27 & 0.09 & 0.36 & 100.00 & 2.52 & 0.15 & 0.27 & 96.00 & 1.33 \\
% \hspace{.15cm} $\text{global}-\ell_1$ & 0.13 & 0.81 & 95.00 & 3.89 & 0.07 & 0.50 & 98.00 & 2.48 & 0.16 & 0.36 & 95.00 & 1.37 \\
% \hspace{.15cm} Fixed-effects & 0.27 & 1.46 & 96.00 & 5.87 & 0.24 & 1.48 & 96.00 & 5.84 & 0.24 & 1.49 & 96.00 & 5.83  \\
\hspace{.15cm} Target-Only & 0.10 & 3.14 & 93.80 & 8.96 & 0.10 & 3.10 & 93.60 & 8.97 & 0.09 & 3.04 & 94.20 & 8.95 \\ 
\hspace{.15cm} SS (naive) & 0.27 & 0.57 & 99.40 & 6.55 & 0.25 & 0.44 & 98.60 & 3.67 & 0.22 & 0.32 & 93.60 & 1.74 \\ 
\hspace{.15cm} SS & 0.24 & 0.57 & 99.80 & 7.01 & 0.22 & 0.42 & 99.00 & 3.84 & 0.19 & 0.29 & 96.80 & 1.79 \\ 
\hspace{.15cm} $\text{global}-\ell_2$ & 0.06 & 0.52 & 99.80 & 6.69 & 0.11 & 0.39 & 99.40 & 3.68 & 0.14 & 0.29 & 95.60 & 1.74 \\ 
\hspace{.15cm} $\text{global}-\ell_1$ & 0.09 & 0.73 & 98.20 & 6.48 & 0.12 & 0.52 & 98.00 & 3.67 & 0.13 & 0.37 & 94.20 & 1.79 \\ 
\hspace{.15cm} Fixed-effects & 0.28 & 1.50 & 93.80 & 5.87 & 0.26 & 1.50 & 93.40 & 5.84 & 0.26 & 1.50 & 94.00 & 5.83 \\ 
\hline
\end{tabular}
Abbreviations: RMSE = Root mean square error; Cov. = Coverage, Len. = Length of $95\%$ CI.
\vspace{.25cm}
\footnotesize{
\begin{flushleft}
\end{flushleft}
}
\end{table}
\end{center}

\subsection*{Weights for the dense covariate setting}
Recall that in the main text, we displayed the $\eta_k$ weights for $k=1,...,K$ when $K=20$ hospitals in the $\mathcal{\text{sparse}}$ setting. Here, we illustrate the $\eta_k$ weights, again for $K = 20$ hospitals, but for the $\mathcal{\text{dense}}$ setting. Figure 3 %\ref{fig:glmnet}
summarizes the results. The $\text{global}-\ell_1$ estimator places about $40\%$ of the weight on the target hospital and drops some sites entirely that have large bias compared to the target site TATE. The SS estimator has the same weights as in the $\mathcal{D}_\text{sparse}$ setting. As in the $\mathcal{D}_\text{sparse}$ setting, the $\text{global}-\ell_2$ estimator produces weights between the $\text{global}-\ell_1$ estimator and the SS estimator. In terms of covariate imbalance, there is less difference between the $\text{global}-\ell_1$ and $\text{global}-\ell_2$ estimators, so the $\text{global}-\ell_2$ estimator may be preferable as it has a larger effective sample size and thus smaller variance since it drops fewer sites. In the $\mathcal{D}_\text{dense}$ setting, the differences in covariate imbalances using the $\text{global}-\ell_1$, $\text{global}-\ell_2$, and SS estimators are less pronounced. In this setting, the $\text{global}-\ell_2$ estimator is preferred to the $\text{global}-\ell_1$ estimator due to its smaller RMSE.
% \begin{figure}[H]
%     \centering
% % \includegraphics[scale = 0.52]{graphics/ss_eta2.pdf} 
% % \includegraphics[scale = 0.52]{graphics/osqp_eta2.pdf}
% % \includegraphics[scale = 0.52]{graphics/glmnet_eta2.pdf} \\
% % \vspace{-0.5cm}
% % \includegraphics[scale = 0.60]{graphics/X2_dense_imbalances.pdf} 
% % \vspace{-0.5cm}
% % \caption{The $\mathcal{D}_{\text{dense}}$ setting where the $\text{global}-\ell_2$ estimator has smaller RMSE, the $\text{global}-\ell_1$ estimator and $\text{global}-\ell_2$ estimator have comparable biases.}
%     \includegraphics[scale=0.75]{graphics/Figure2S_A.pdf}
%     \includegraphics[scale=0.75]{graphics/Figure2S_B.pdf}
%     \caption{At left, we plot the distance from each source hospital to the target TATE vs. hospital weights in the $\mathcal{D}_{\text{dense}}$ setting, showing the GLOBAL estimators upweight hospitals with similar TATE estimates. At right, we observe smaller covariate imbalances between the target and source hospitals when using the GLOBAL estimators.}
%     \label{fig:osqp}
% \end{figure}

% \section*{Appendix IV. Example of Covariate Imbalance in the CCE Analysis}
% To illustrate the covariate imbalances using the ss, global-$\ell_1$, and global-$\ell_2$ estimators, we plot the imbalances of two covariates (proportion of female vs. proportion of anterior myocardial infarctions), where each dot represents one of the $51$ hospitals being the target of interest. The results show that the global-$\ell_1$ estimator has the smallest covariate imbalances, followed by the global-$\ell_2$ estimator, with the ss estimator displaying the largest covariate imbalance.

% \begin{figure}[H]
% \begin{center}
% \includegraphics[scale = 0.7]{graphics/imb_case.pdf} 
% \end{center}
% \vspace{-0.5cm}
%     \caption{Imbalances of two covariates (proportion of female patients vs proportion of patients admitted with anterior myocardial infarctions) for all 51 hospitals. Each dot represents one of the hospitals serving as a target hospital. ({\color{red} to be updated})}
%     \label{fig:weights}
% \end{figure}


% \newpage
% \section*{Appendix IV. Hospital Characteristics}

% \begin{center}
% \renewcommand{\arraystretch}{0.7}
% \begin{table}[H]
% \caption{Comparison of the estimates (LOS)}
% \centering
% \tiny
% \setlength{\tabcolsep}{2pt}
% \begin{tabular}{lrrrrrrrrrrrr}
%   \hline
%   & \multicolumn{12}{c}{Estimates} \\
%      \cmidrule(lr){2-13} 
%   &  \multicolumn{4}{c}{$\E[Y(\text{PCI})]$} &  \multicolumn{4}{c}{$\E[Y(\text{MM})]$} &  \multicolumn{4}{c}{ATE} \\
%   %&  \multicolumn{4}{c}{$K = 100$} \\
%   \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17}
%       & Raw & Target & Indirect & Direct & Raw & Target & Indirect & Direct & Raw & Target & Indirect & Direct\\
%   \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17}
% Distribution &  &  &\\ 
% \hspace{.15cm} 0\% & 4.17 & 4.08 & 4.45 & 4.71 & 5.90 & 5.85 & 6.23 & 6.50 & -7.00 & -6.24 & -4.45 & -4.06 \\ 
% \hspace{.15cm}  25\% & 5.17 & 5.30 & 5.16 & 5.14 & 7.74 & 7.74 & 7.29 & 7.25 & -3.44 & -3.34 & -2.85 & -2.72 \\ 
% \hspace{.15cm}  50\% & 5.84 & 5.87 & 5.35 & 5.32 & 8.25 & 8.33 & 7.71 & 7.73 & -2.64 & -2.56 & -2.42 & -2.38 \\ 
% \hspace{.15cm}  75\% & 6.47 & 6.59 & 5.59 & 5.61 & 9.34 & 9.30 & 8.23 & 8.21 & -1.92 & -1.64 & -1.86 & -1.94 \\ 
% \hspace{.15cm}  100\% & 7.94 & 8.89 & 6.25 & 6.35 & 12.10 & 11.51 & 9.97 & 9.52 & 0.95 & 1.01 & -0.40 & -0.15 \\ 
%   \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13}
%   Hospital \\
% \hspace{.15cm} A & 7.43 & 7.55 & 6.10 & 5.73 & 10.25 & 10.14 & 8.58 & 8.20 & -2.82 & -2.58 & -2.48 & -2.47 \\ 
% \hspace{.15cm} B & 4.33 & 4.08 & 4.45 & 4.85 & 7.51 & 7.45 & 7.33 & 7.41 & -3.18 & -3.37 & -2.88 & -2.56 \\ 
% \hspace{.15cm} C & 6.52 & 6.91 & 5.71 & 5.65 & 8.39 & 7.91 & 7.42 & 7.25 & -1.87 & -0.99 & -1.71 & -1.60 \\ 
% \hspace{.15cm} Top 5 Avg. & 4.46 & 4.64 & 4.80 & 4.90 & 6.32 & 6.19 & 6.50 & 6.75 & -5.29 & -4.89 & -3.72 & -3.66 \\ 
% \hspace{.15cm} Bottom 5 Avg. & 7.55 & 7.96 & 6.13 & 5.97 & 11.01 & 10.83 & 8.95 & 8.96 & 0.05 & 0.34 & -1.04 & -1.03 \\
%   \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} %\cmidrule(lr){14-17}
% Specification I &  &  &\\ 
% %$n_k = 100$ &  &  &\\ 
% \hspace{.15cm} Intercept & 5.87(0.91) & 6.04(0.98) & 5.40(0.37) & 5.37(0.32) & 8.50(1.33) & 8.49(1.34) & 7.73(0.72) & 7.72(0.66) & -2.63(1.49) & -2.45(1.49) & -2.33(0.76) & -2.35(0.73) \\
%   \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13}
% Specification II &  &  &\\ 
% \hspace{.15cm} Intercept & 5.71(0.14) & 5.85(0.15) & 5.36(0.06) & 5.36(0.05) & 8.28(0.21) & 8.28(0.21) & 7.66(0.12) & 7.61(0.10) &  -2.57(0.25) & -2.42(0.25) & -2.30(0.13) & -2.26(0.12) \\
% \hspace{.15cm} Bed count $>$ 800 &  *0.58(0.28) & *0.70(0.29) & 0.12(0.12) & 0.06(0.10) & 0.79(0.41) & 0.78(0.41) & 0.23(0.23) & *0.41(0.20) & -0.21(0.47) & -0.08(0.47) & -0.11(0.24) & -0.35(0.23)\\
%   \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
% Specification III &  &  &\\ 
% %$n_k = 100$ &  &  &\\ 
% \hspace{.15cm} Intercept & 5.75(0.18) &  5.89(0.19)    & 5.32(0.07) & 5.33(0.06) & 8.22(0.26)  & 8.15(0.26)    & 7.55(0.14)  &   7.68(0.13) &   -2.47(0.29) & -2.26(0.29) &   -2.23(0.15)  &  -2.35(0.14)\\
% \hspace{.15cm} NTB $>$ Median &  0.24(0.26) & 0.32(0.27) & 0.15(0.10) & 0.09(0.09) & 0.57(0.37) &  0.70(0.36)  &   0.35(0.20)  &   0.09(0.19)  &  -0.33(0.42) & -0.38(0.42) &   -0.20(0.21)  &  -0.01(0.21)\\
%   \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} Specification III &  &  &\\ 
% %$n_k = 100$ &  &  &\\ 
% \hspace{.15cm} Intercept & 5.60(0.19) & 5.70(0.20) & 5.29(0.08) & 5.31(0.07) & 8.01(0.27) & 7.94(0.27) & 7.49(0.15) & 7.57(0.14) & -2.41(0.32) & -2.24(0.32) & -2.20(0.16) & -2.25(0.16) \\
% \hspace{.15cm} Bed count $>$ 800 &  *0.58(0.28) & *0.69(0.29) & 0.12(0.12) & 0.06(0.10) & 0.78(0.40) & 0.77(0.40) & 0.22(0.22) & *0.41(0.20) & -0.21(0.47) & -0.07(0.47) & -0.10(0.24) & -0.35(0.23)\\
% \hspace{.15cm} NTB $>$ Median & 0.23(0.25) & 0.31(0.26) & 0.15(0.10) & 0.09(0.09) & 0.56(0.36) & 0.69(0.36) & 0.35(0.20) & 0.09(0.18) & -0.33(0.42) & -0.38(0.42) & -0.20(0.21) & -0.00(0.20) \\ 
% \hline
% \end{tabular}
% \vspace{.25cm}
% \footnotesize{
% \begin{flushleft}
% \end{flushleft}
% }
% \end{table}
% \end{center}



% \begin{center}
% \renewcommand{\arraystretch}{0.7}
% \begin{table}[H]
% \caption{Comparison of the estimates (Mortality) NFP are getting older patient for MM but not for PCI}
% \centering
% \tiny
% \setlength{\tabcolsep}{2pt}
% \begin{tabular}{lrrrrrrrrrrrr}
%   \hline
%   & \multicolumn{12}{c}{Estimates} \\
%      \cmidrule(lr){2-13} 
%   &  \multicolumn{4}{c}{$\E[Y(\text{PCI})]$} &  \multicolumn{4}{c}{$\E[Y(\text{MM})]$} &  \multicolumn{4}{c}{ATE} \\
%   %&  \multicolumn{4}{c}{$K = 100$} \\
%   \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
%       & Raw & Target & Indirect & Direct & Raw & Target & Indirect & Direct & Raw & Target & Indirect & Direct\\
%   \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13}
% Distribution &  &  &\\ 
% \hspace{.15cm}  0\% & 0.00 & -1.21 & 0.11 & -0.50 & 6.25 & 2.04 & 5.53 & 2.97 & -21.32 & -14.44 & -11.86 & -8.91 \\
% \hspace{.15cm}  25\% & 3.70 & 3.48 & 2.42 & 1.99 & 11.15 & 9.40 & 7.36 & 7.00 & -9.46 & -8.58 & -6.74 & -6.70 \\ 
% \hspace{.15cm}  50\% & 5.93 & 6.00 & 3.25 & 2.83 & 12.69 & 11.54 & 9.23 & 8.68 & -7.52 & -5.09 & -4.87 & -5.65 \\ 
% \hspace{.15cm}  75\% & 7.77 & 8.79 & 5.80 & 3.98 & 15.17 & 13.85 & 10.35 & 10.16 & -4.89 & -2.67 & -3.64 & -4.75 \\ 
% \hspace{.15cm}  100\% & 10.34 & 10.96 & 9.83 & 5.81 & 26.32 & 24.74 & 13.65 & 13.78 & 1.59 & 7.59 & 1.11 & -2.96 \\ 
% \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
% Specification I &  &  &\\ 
% %$n_k = 100$ &  &  &\\ 
% \hspace{.15cm} Intercept &  5.71(0.34) & 6.04(0.43) & 4.01(0.29) & 2.88(0.20) & 13.28(0.52) & 11.70(0.55) & 9.08(0.27) & 8.60(0.36) & -7.57(0.62) & -5.66(0.68) & -5.07(0.38) & -5.72(0.20) \\ 
%   \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13}
% Specification II &  &  &\\ 
% \hspace{.15cm} Intercept & 5.77(0.41) & 5.79(0.51) & 3.91(0.34) & 2.91(0.24) & 12.90(0.61) & 11.03(0.63) & 8.70(0.31) & 8.56(0.43) & -7.13(0.73) & -5.24(0.80) & -4.79(0.45) & -5.66(0.24) \\
% \hspace{.15cm} Bed count $>$ 800 & -0.23(0.78) & 0.91(0.97) & 0.37(0.64) & -0.09(0.45) & 1.39(1.16) & *2.41(1.20) & *1.39(0.59) & 0.15(0.82) & -1.62(1.39) & -1.50(1.53) & -1.02(0.85) & -0.24(0.45) \\ 
% \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13}
% Specification II' &  &  &\\ 
% \hspace{.15cm} Intercept & 6.27(0.51) & 7.08(0.62) & 4.80(0.40) & 3.17(0.30) & 13.18(0.78) & 11.79(0.83) & 9.05(0.41) & 8.90(0.54) & -6.91(0.93) & -4.72(1.01) & -4.25(0.55) & -5.73(0.30) \\
% \hspace{.15cm} Teaching & -1.03(0.68) & *-1.89(0.84) & *-1.44(0.54) & -0.53(0.40) & 0.18(1.06) & -0.17(1.12) & 0.06(0.56) & -0.54(0.73) & -1.21(1.25) & -1.71(1.37) & *-1.50(0.74) & 0.01(0.41) \\
%   \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
% Specification II'' &  &  &\\
% \hspace{.15cm} Intercept & 6.27(0.48) & 7.23(0.58) & 4.43(0.40) & 3.15(0.28) & 13.11(0.75) & 11.75(0.79) & 8.48(0.38) & 9.13(0.51) & -6.84(0.89) & -4.53(0.96) & -4.05(0.51) & -5.98(0.28) \\
% \hspace{.15cm} owner\_nfp & -1.11(0.68) & *-2.33(0.81) & -0.82(0.57) & -0.52(0.40) & 0.33(1.05) & -0.11(1.11) & *1.18(0.53) & -1.03(0.72) & -1.44(1.24) & -2.22(1.34) & *-2.00(0.72) & 0.51(0.40) \\
% \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13}
% Specification III &  &  &\\ 
% %$n_k = 100$ &  &  &\\ 
% \hspace{.15cm} Intercept & 5.57(0.49) & 5.69(0.61) & 3.92(0.40) & 2.78(0.28) & 13.09(0.73) & 11.46(0.78) & 8.75(0.38) & 8.48(0.51) & -7.52(0.88) & -5.78(0.97) & -4.83(0.54) & -5.69(0.28) \\ 
% \hspace{.15cm} NTB $>$ Median & 0.28(0.69) & 0.72(0.87) & 0.18(0.58) & 0.19(0.40) & 0.39(1.05) & 0.47(1.11) & 0.66(0.54) & 0.25(0.73) & -0.11(1.26) & 0.25(1.38) & -0.48(0.77) & -0.06(0.40) \\ 
%   \cmidrule(lr){1-1}  \cmidrule(lr){2-5}  \cmidrule(lr){6-9} \cmidrule(lr){10-13} Specification III &  &  &\\ 
% %$n_k = 100$ &  &  &\\ 
% \hspace{.15cm} Intercept & 5.63(0.53) & 5.44(0.66) & 3.82(0.44) & 2.81(0.31) & 12.72(0.80) & 10.82(0.82) & 8.38(0.40) & 8.44(0.56) & -7.09(0.96) & -5.37(1.05) & -4.56(0.58) & -5.63(0.31) \\ 
% \hspace{.15cm} Bed count $>$ 800 & -0.23(0.78) & 0.90(0.98) & 0.37(0.65) & -0.10(0.46) & 1.38(1.17) & *2.41(1.21) & *1.38(0.58) & 0.14(0.83) & -1.62(1.40) & -1.51(1.55) & -1.01(0.86) & -0.24(0.46) \\ 
% \hspace{.15cm} NTB $>$ Median & 0.28(0.70) & 0.71(0.87) & 0.18(0.58) & 0.20(0.41) & 0.37(1.05) & 0.45(1.08) & 0.65(0.52) & 0.25(0.74) & -0.09(1.25) & 0.26(1.38) & -0.47(0.77) & -0.06(0.41) \\ 
% \hline
% \end{tabular}
% \vspace{.25cm}
% \footnotesize{
% \begin{flushleft}
% \end{flushleft}
% }
% \end{table}
% \end{center}


\clearpage
\section*{Appendix IV. Additional Real Data Analysis Results}

\subsection*{Covariate Balance Diagnostics}
In addition to 30-day mortality, we also study the causal effect of PCI versus MM on patient length of stay. Detailed covariate balance diagnostics for indirect standardization and direct standardization are provided in the tables below.

\begin{table}[ht]
\centering
\caption{Covariate balance diagnostics for LOS as the outcome (indirect standardization)}
\scriptsize
\setlength{\tabcolsep}{1pt}
\begin{tabular}{lrrrrrrrrr}
  \hline
Hospital A & Goal & Hosp A PCI & Hosp A MM & Source PCI & Source MM & Tgt-Only PCI & Tgt-Only MM & Global-$\ell_1$ PCI & Global-$\ell_1$ MM \\  
  \hline
Covariates \\
\hspace{.15cm} Age & 80.52 & 79.11 & 81.67 & 76.52 & 79.24 & 80.52 & 80.52 & 80.52 & 80.52 \\ 
\hspace{.15cm} Female & 0.45 & 0.38 & 0.51 & 0.41 & 0.46 & 0.45 & 0.45 & 0.45 & 0.45 \\ 
\hspace{.15cm} History of PCI & 0.23 & 0.28 & 0.19 & 0.23 & 0.22 & 0.23 & 0.23 & 0.23 & 0.23 \\ 
\hspace{.15cm} Renal Disease & 0.45 & 0.43 & 0.47 & 0.29 & 0.45 & 0.45 & 0.45 & 0.45 & 0.45 \\ 
  Eff. sample size &  & 81 & 100 & 4923 & 5999 & 68 & 51 & 1321 & 1818 \\ 
  \hline
Hospital B & Goal & Hosp A PCI & Hosp A MM & Source PCI & Source MM & Tgt-Only PCI & Tgt-Only MM & Global-$\ell_1$ PCI & Global-$\ell_1$ MM \\  
  \hline
Covariates \\
\hspace{.15cm} Age & 75.89 & 75.56 & 76.12 & 76.58 & 79.34 & 75.89 & 75.89 & 75.89 & 75.89 \\ 
\hspace{.15cm} Female & 0.36 & 0.33 & 0.38 & 0.41 & 0.46 & 0.36 & 0.36 & 0.36 & 0.36 \\ 
\hspace{.15cm} History of PCI & 0.18 & 0.18 & 0.18 & 0.24 & 0.22 & 0.18 & 0.18 & 0.18 & 0.18 \\ 
\hspace{.15cm} Renal Disease & 0.32 & 0.29 & 0.34 & 0.30 & 0.45 & 0.32 & 0.32 & 0.32 & 0.32 \\ 
  Eff. sample size &  & 91 & 128 & 4913 & 5971 & 76 & 110 & 1475 & 1349 \\ 
   \hline
Hospital C & Goal & Hosp A PCI & Hosp A MM & Source PCI & Source MM & Tgt-Only PCI & Tgt-Only MM & Global-$\ell_1$ PCI & Global-$\ell_1$ MM \\  
  \hline
Covariates \\
\hspace{.15cm} Age & 78.70 & 77.02 & 80.35 & 76.56 & 79.26 & 78.70 & 78.70 & 78.70 & 78.70 \\ 
\hspace{.15cm} Female & 0.49 & 0.49 & 0.48 & 0.40 & 0.46 & 0.49 & 0.49 & 0.49 & 0.49 \\ 
\hspace{.15cm} History of PCI & 0.25 & 0.25 & 0.24 & 0.23 & 0.21 & 0.25 & 0.25 & 0.25 & 0.25 \\ 
\hspace{.15cm}  Renal Disease & 0.40 & 0.30 & 0.50 & 0.29 & 0.45 & 0.40 & 0.40 & 0.40 & 0.40 \\ 
  Eff. sample size &  & 87 & 88 & 4917 & 6011 & 72 & 60 & 1357 & 1415 \\ 
   \hline
\end{tabular}
\end{table}


\begin{table}[ht]
\centering
\caption{Covariate balance diagnostics for LOS as the outcome (direct standardization)}
\scriptsize
\setlength{\tabcolsep}{1pt}
\begin{tabular}{lrrrrrrrrr}
  \hline
Hospital A & Goal & Hosp A PCI & Hosp A MM & Source PCI & Source MM & Tgt-Only PCI & Tgt-Only MM & Global-$\ell_1$ PCI & Global-$\ell_1$ MM \\  
  \hline
Covariates \\
\hspace{.15cm} Age & 78.05 & 79.11 & 81.67 & 76.52 & 79.24 & 78.05 & 78.05 & 78.05 & 78.05 \\ 
\hspace{.15cm} Female & 0.44 & 0.38 & 0.51 & 0.41 & 0.46 & 0.44 & 0.44 & 0.44 & 0.44 \\ 
\hspace{.15cm} History of PCI & 0.22 & 0.28 & 0.19 & 0.23 & 0.22 & 0.22 & 0.22 & 0.22 & 0.22 \\ 
\hspace{.15cm} Renal Disease & 0.38 & 0.43 & 0.47 & 0.29 & 0.45 & 0.38 & 0.38 & 0.38 & 0.38 \\ 
Eff. sample size &  & 81 & 100 & 4923 & 5999 & 69 & 45 & 1660 & 1609 \\ 
  \hline
Hospital B & Goal & Hosp A PCI & Hosp A MM & Source PCI & Source MM & Tgt-Only PCI & Tgt-Only MM & Global-$\ell_1$ PCI & Global-$\ell_1$ MM \\  
  \hline
Covariates \\
\hspace{.15cm} Age & 78.05 & 75.56 & 76.12 & 76.58 & 79.34 & 78.05 & 78.05 & 78.05 & 78.05 \\ 
\hspace{.15cm} Female & 0.44 & 0.33 & 0.38 & 0.41 & 0.46 & 0.44 & 0.44 & 0.44 & 0.44 \\ 
\hspace{.15cm} History of PCI & 0.22 & 0.18 & 0.18 & 0.24 & 0.22 & 0.22 & 0.22 & 0.22 & 0.22 \\ 
\hspace{.15cm} Renal Disease & 0.38 & 0.29 & 0.34 & 0.30 & 0.45 & 0.38 & 0.38 & 0.38 & 0.38 \\ 
Eff. sample size &  & 91 & 128 & 4913 & 5971 & 60 & 92 & 1606 & 1709 \\ 
   \hline
Hospital C & Goal & Hosp A PCI & Hosp A MM & Source PCI & Source MM & Tgt-Only PCI & Tgt-Only MM & Global-$\ell_1$ PCI & Global-$\ell_1$ MM \\  
  \hline
Covariates \\
\hspace{.15cm} Age & 78.05 & 77.02 & 80.35 & 76.56 & 79.26 & 78.05 & 78.05 & 78.05 & 78.05 \\ 
\hspace{.15cm} Female & 0.44 & 0.49 & 0.48 & 0.40 & 0.46 & 0.44 & 0.44 & 0.44 & 0.44 \\ 
\hspace{.15cm} History of PCI & 0.22 & 0.25 & 0.24 & 0.23 & 0.21 & 0.22 & 0.22 & 0.22 & 0.22 \\ 
\hspace{.15cm} Renal Disease & 0.38 & 0.30 & 0.50 & 0.29 & 0.45 & 0.38 & 0.38 & 0.38 & 0.38 \\ 
Eff. sample size  &  & 87 & 88 & 4917 & 6011 & 67 & 47 & 1345 & 1266 \\ 
   \hline
\end{tabular}
\end{table}


\subsection*{Causal Effect of PCI versus MM on Length of Stay}
We illustrate that there is again a marked difference in hospital weights $\boldsymbol{\eta}$ using our proposed global estimators GLOBAL-$\ell_1$ and GLOBAL-$\ell_2$ compared to SS. As before, we showcase our method with the same three diverse target hospitals. GLOBAL-$\ell_1$ places more weight on hospitals with relatively small bias, while GLOBAL-$\ell_2$ is in between GLOBAL-$\ell_1$ and the SS estimator as before. Interestingly, there is not as clear of a monotonic decreasing relationship between bias and hospital weight as in the case of 30-day mortality.

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.31]{graphics/Figure5_dist_plots_los_indirect_same_1209.PDF}
    \caption{LOS: The global estimators place more weight on source hospitals with more similar estimates regardless of estimand, whether the target hospital is an urban major teaching hospital (A), an urban for-profit hospital (B), or a rural non-teaching hospital (C).}
    \label{fig:fig3los}
\end{figure}

The causal effect of PCI versus MM on LOS was negative and statistically significant in $90\%$ of the hospitals using our GLOBAL-$\ell_1$ estimator, compared to just 59\% using the target-only estimator. The  TATE is measured in days, showing that patients treated with PCI tended to have a shorter average LOS compared to MM by approximately $2$ to $4$ days. Relative to the target-only estimator, the percent reduction in the $95\%$ CI length with the GLOBAL-$\ell_1$ estimator ranged from $65\%$ to $87\%$ with a median of $80\%$. With this increased precision, $31\%$ ($16/51$) of hospitals had a qualitative change in the causal effect of PCI on shorter LOS from not statistically significant to statistically significantly shorter.

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.31]{graphics/Figure8_ATE_all_los_indirect_1130.PDF}
    \caption{LOS: TATE estimates for all $51$ hospitals show substantial precision gain of GLOBAL-$\ell_1$ compared to the Target-Only estimator and accuracy comparable to the GLOBAL-$\ell_2$ and SS estimators.}
    \label{fig:fig4los}
\end{figure}


Figure \ref{fig:fig5los} shows hospital LOS estimates for PCI and MM, with hospitals sequenced from the lowest (best) to highest (worst) PCI LOS. We find that PCI patients had shorter LOS than MM patients in all hospitals. As with 30-day mortality, very few hospitals fared particularly well on both PCI and MM rankings for LOS. 


\begin{figure}[H]
    \centering
    \includegraphics[scale=0.5]{graphics/Figure10_spine_plots_by_tx_los_indirect_1130.PDF}
    \caption{LOS: GLOBAL-$\ell_1$ hospital mortality estimates and $95\%$ CIs show that hospitals that ranked highly on PCI mortality tended not to rank as well on MM and vice versa; moreover, MM mortality estimates varied considerably even among hospitals with similar PCI performance.}
    \label{fig:fig5los}
\end{figure}


% \begin{table}[ht]
% \centering
% \caption{Means of age averages of patients under PCI and MM over each hospital ownership}
% \begin{tabular}{lrrrr}
%   \hline
%  & All & PCI & MM & Diff\\ 
%   \hline
% nfp & 78.40 & 76.60 & 79.83 & 3.23 \\ 
% for-profit & 77.42 & 76.55 & 78.11 & 1.56\\ 
% government & 76.72 & 75.78 & 77.51 & 1.73 \\ 
% hosp district & 77.23 & 75.85 & 78.16 & 2.30 \\ 
% other & 78.56 & 77.10 & 79.83 & 2.73 \\ 
% physician & 78.36 & 77.78 & 79.02 & 1.24\\ 
% religious & 77.99 & 76.67 & 79.11 & 2.44\\ 
%   \hline
% \end{tabular}
% \end{table}

% \begin{table}[ht]
% \centering
% \caption{Age differences between patients under PCI and patients under MM, comparing the other hospital ownership to NFP}
% \begin{tabular}{lrrrr}
%   \hline
%  & Estimate & Std. Error & t-value & p-value \\ 
%   \hline
% nfp & 3.23 & 0.21 & 15.45 & 0.00 \\ 
%   for-profit & -1.67 & 0.52 & -3.21 & 0.00 \\ 
%   government & -1.50 & 0.65 & -2.30 & 0.03 \\ 
%   hosp district & -0.93 & 0.65 & -1.42 & 0.16 \\ 
%   other & -0.50 & 0.43 & -1.17 & 0.25 \\ 
%   physician & -1.99 & 1.09 & -1.83 & 0.07 \\ 
%   religious & -0.79 & 0.52 & -1.53 & 0.13 \\ 
%   \hline
% \end{tabular}
% \end{table}

% \newpage
% \begin{figure}[H]
% \begin{center}
% \includegraphics[scale = 0.3]{graphics/Mortality_direct_mu_all.pdf} 
% \includegraphics[scale = 0.3]{graphics/Mortality_direct_mu1_methods.pdf} 
% \includegraphics[scale = 0.3]{graphics/Mortality_direct_mu0_methods.pdf} 
% \includegraphics[scale = 0.3]{graphics/Mortality_indirect_mu_all.pdf} 
% \includegraphics[scale = 0.3]{graphics/Mortality_indirect_mu1_methods.pdf} 
% \includegraphics[scale = 0.3]{graphics/Mortality_indirect_mu0_methods.pdf} 
% \includegraphics[scale = 0.3]{graphics/LOS_direct_mu_all.pdf} 
% \includegraphics[scale = 0.3]{graphics/LOS_direct_mu1_methods.pdf} 
% \includegraphics[scale = 0.3]{graphics/LOS_direct_mu0_methods.pdf} 
% \includegraphics[scale = 0.3]{graphics/LOS_indirect_mu_all.pdf} 
% \includegraphics[scale = 0.3]{graphics/LOS_indirect_mu1_methods.pdf} 
% \includegraphics[scale = 0.3]{graphics/LOS_indirect_mu0_methods.pdf} 
% \caption{Old version - shared outcome model, shrink too much}
% \end{center}
% \end{figure}

% \begin{figure}[H]
% \begin{center}
% \includegraphics[scale = 0.3]{graphics_temp/Mortality_direct_mu_all_intercept.pdf} 
% \includegraphics[scale = 0.3]{graphics_temp/Mortality_direct_mu1_methods_intercept.pdf} 
% \includegraphics[scale = 0.3]{graphics_temp/Mortality_direct_mu0_methods_intercept.pdf} 
% \includegraphics[scale = 0.3]{graphics_temp/Mortality_indirect_mu_all_intercept.pdf} 
% \includegraphics[scale = 0.3]{graphics_temp/Mortality_indirect_mu1_methods_intercept.pdf} 
% \includegraphics[scale = 0.3]{graphics_temp/Mortality_indirect_mu0_methods_intercept.pdf} 
% \includegraphics[scale = 0.3]{graphics_temp/LOS_direct_mu_all.pdf} 
% \includegraphics[scale = 0.3]{graphics_temp/LOS_direct_mu1_methods.pdf} 
% \includegraphics[scale = 0.3]{graphics_temp/LOS_direct_mu0_methods.pdf} 
% \includegraphics[scale = 0.3]{graphics_temp/LOS_indirect_mu_all.pdf} 
% \includegraphics[scale = 0.3]{graphics_temp/LOS_indirect_mu1_methods.pdf} 
% \includegraphics[scale = 0.3]{graphics_temp/LOS_indirect_mu0_methods.pdf} 
% \caption{New version - outcome models with vary parameters, shrink less}
% \end{center}
% \end{figure}

% \begin{figure}[H]
% \begin{center}
% \includegraphics[scale = 0.45]{graphics_temp2/Mortality_direct_mu1_methods_intercept.pdf} 
% \includegraphics[scale = 0.45]{graphics_temp2/Mortality_direct_mu0_methods_intercept.pdf} 
% \includegraphics[scale = 0.45]{graphics_temp2/Mortality_indirect_mu1_methods_intercept.pdf} 
% \includegraphics[scale = 0.45]{graphics_temp2/Mortality_indirect_mu0_methods_intercept.pdf} 
% \caption{Latest version - outcome models with vary parameters, adaptive tuning algorithm, shrink less}
% \end{center}
% \end{figure}

% \newpage
% \begin{figure}[H]
% \begin{center}
% \includegraphics[scale = 0.45]{graphics_temp/LOS_indirect_mu1_verify.pdf} 
% \includegraphics[scale = 0.45]{graphics_temp/LOS_indirect_mu0_verify.pdf} 
% \caption{Verification with fixed targets}
% \end{center}
% \end{figure}


% \newpage
% \begin{figure}[H]
% \begin{center}
% \begin{subfigure}{0.99\textwidth}
% \includegraphics[scale = 0.225]{graphics/Mortality_direct_eta1_glmnet.pdf} 
% \includegraphics[scale = 0.225]{graphics/Mortality_direct_eta1_osqp.pdf} 
% \includegraphics[scale = 0.225]{graphics/Mortality_direct_eta0_glmnet.pdf} 
% \includegraphics[scale = 0.225]{graphics/Mortality_direct_eta0_osqp.pdf}
% \caption{Mortality, Direct, ($\mu_1 (\ell_1)$, $\mu_1 (\ell_2)$, $\mu_0 (\ell_1)$, $\mu_0 (\ell_2)$)}
% \end{subfigure}
% \begin{subfigure}{0.99\textwidth}
% \includegraphics[scale = 0.225]{graphics/Mortality_indirect_eta1_glmnet.pdf} 
% \includegraphics[scale = 0.225]{graphics/Mortality_indirect_eta1_osqp.pdf} 
% \includegraphics[scale = 0.225]{graphics/Mortality_indirect_eta0_glmnet.pdf} 
% \includegraphics[scale = 0.225]{graphics/Mortality_indirect_eta0_osqp.pdf} 
% \caption{Mortality, Indirect, ($\mu_1 (\ell_1)$, $\mu_1 (\ell_2)$, $\mu_0 (\ell_1)$, $\mu_0 (\ell_2)$)}
% \end{subfigure}
% \begin{subfigure}{0.99\textwidth}
% \includegraphics[scale = 0.225]{graphics/LOS_direct_eta1_glmnet.pdf} 
% \includegraphics[scale = 0.225]{graphics/LOS_direct_eta1_osqp.pdf} 
% \includegraphics[scale = 0.225]{graphics/LOS_direct_eta0_glmnet.pdf} 
% \includegraphics[scale = 0.225]{graphics/LOS_direct_eta0_osqp.pdf} 
% \caption{LOS, Direct, ($\mu_1 (\ell_1)$, $\mu_1 (\ell_2)$, $\mu_0 (\ell_1)$, $\mu_0 (\ell_2)$)}
% \end{subfigure}
% \begin{subfigure}{0.99\textwidth}
% \includegraphics[scale = 0.225]{graphics/LOS_indirect_eta1_glmnet.pdf} 
% \includegraphics[scale = 0.225]{graphics/LOS_indirect_eta1_osqp.pdf} 
% \includegraphics[scale = 0.225]{graphics/LOS_indirect_eta0_glmnet.pdf} 
% \includegraphics[scale = 0.225]{graphics/LOS_indirect_eta0_osqp.pdf} 
% \caption{LOS, Indirect, ($\mu_1 (\ell_1)$, $\mu_1 (\ell_2)$, $\mu_0 (\ell_1)$, $\mu_0 (\ell_2)$)}
% \end{subfigure}
% \end{center}
% \end{figure}

